On sets of numbers rationally represented in a rational base number system

In this work, it is proved that a set of numbers closed under addition and whose representations in a rational base numeration system is a rational language is not a finitely generated additive monoid. A key to the proof is the definition of a strong combinatorial property on languages : the bounded left iteration property. It is both an unnatural property in usual formal language theory (as it contradicts any kind of pumping lemma) and an ideal fit to the languages defined through rational base number systems.

==> VCPref-beamer.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Package `VauCanSon-G'  version 0.4
%%
%% This is file `VCPref-slides'.
%%
%% IMPORTANT NOTICE:
%%
%% Copyright (C) 2002-2008 Sylvain Lombardy and Jacques Sakarovitch
%%
%% This package may be distributed under the terms of the LaTeX Project
%% Public License, as described in lppl.txt in the base LaTeX distribution.
%% Either version 1.0 or, at your option, any later version.
%%
%% DESCRIPTION:
%%
%%   `VCPref-beamer' contains initial values of VauCanSon-G 
%%   parameters suitable for drawing automata in slides.
%%   Works with package `beamer'; 
%%   smaller scale values than those given in `VCPref-slides'
%%  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scales  --- slides settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\LargeScale}{0.85}       
\renewcommand{\MediumScale}{0.6}       
\renewcommand{\SmallScale}{0.4}		
\renewcommand{\TinyScale}{0.30}		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% State aspect
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetStateLineColor{blue}
\SetStateLineWidth{2pt}
\SetStateFillColor{Cyan}
\SetStateLabelColor{Sepia}
\FixDimState{solid}{YellowOrange}{1}{YellowOrange}{white}
%%%%%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetEdgeLineColor{Mahogany}
\SetEdgeLineWidth{1.2pt}
\SetEdgeLabelColor{OliveGreen}
%%% Dimmed edges
\FixDimEdge{dashed}{1.2}{Apricot}{Apricot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput


==> VCPref-mystyle.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:    VCPref-mystyle
%%
%% DESCRIPTION:  personal setting of VauCanSon-G's parameters
%%
%  By definiton, an empty file to be customised.
%  
%  VCSG-Preferences.tex is copied after the \endinput
%  andcan be used as a template to write 
%  a customized style of Vaucanson.
%  
%%  
%% DATE:    2012/07/05
%%
%% Copyright (C) 2009-2012 Sylvain Lombardy and Jacques Sakarovitch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-environment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Scaling matters}%%%%%  
% Inner parameters
\renewcommand{\LargeScale}{0.85}    %float : argument of a \scalebox
\renewcommand{\LargeScaleI}{1.18}
\renewcommand{\MediumScale}{0.6}    %float
\renewcommand{\MediumScaleI}{1.67}
\renewcommand{\SmallScale}{0.5}     %float
\renewcommand{\SmallScaleI}{2}
\renewcommand{\TinyScale}{0.42}     %float
\renewcommand{\TinyScaleI}{2.38}
%
\MediumPictures
\FixVCGridScale{1}
%%%%%\section{Picture directory}%%%%%
% \SetVCDirectory{}  % for record : the definition of \VCDirectory is 
%                    % an initialisation 
%%%%%\section{Picture framing}%%%%%
% Inner parameters
\setlength{\VCFrameLineWidth}{0.6pt}
\renewcommand{\VCFrameLineColor}{black}
\setlength{\VCGridLineWidth}{0.6pt}
\renewcommand{\VCGridLineColor}{black}
%
\SetVCBkgdStyle{solid} % Also set StateBkgd, SmallStateBkgd,
                       % SttBorderColor,EdgeLineBorderColor
\SetVCBkgdColor{white} % and DblEdgeLineColor
%
\HideFrame\HideGrid\HideName
%%%%%\section{Picture drawing call}%%%%%
\FixVerticalPlacement{0.5} %float 
%%%%%\section{VauCanSon-G modes}%%%%%
\Automata 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-states}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{node mode}%%%%%%
% \SizedNodes % for record; not necessary after the call to \Automata 
%%%%%\section{state size}%%%%%%
\setlength{\SmallStateDiameter}{.6cm}
\setlength{\MediumStateDiameter}{1cm}
\setlength{\LargeStateDiameter}{1.2cm}
% \FixStateSizes{.6cm}{.9cm}{1.2cm}{.3cm} would have the same effect
%
% \MediumStates postponed after the definition of loop geometry 
% parameters
%%%%%\section{state shape}%%%%%
\CircleStates
\SetOvalStateRatio{\GoldMeanI}
\SetRectangleStateRatio{\GoldMeanI}
%
\SharpStateCorners 
\StateCornerRoundingAbsolute
\SetStateCornerRelRadius{0}
\SetStateCornerRadius{0.2cm}
%%%%%\section{Hiding -- showing}%%%%%
\ShowStates
%%%%%\section{state background parameters}%%%%%
% for record: setting done when setting the Bkgd of the picture 
% \SetStateBkgdStyle{\VCBkgdStyle}\SetStateBkgdColor{\VCBkgdColor}
% \SetSmallStateBkgdStyle{\VCBkgdStyle}
% \SetSmallStateBkgdColor{\VCBkgdColor}
%%%%%\section{construction line parameters}%%%%%%
\renewcommand{\SqrSttCtrClr}{blue}
\renewcommand{\LblBxLnClr}{red}
\renewcommand{\PhtSttLnClr}{green}
\CtrBxLblOff
\CtrSqrSttOff
\CtrPhtSttOff
\setlength{\PhtSttCtr}{0pt} %%% 
%%%%%\section{state line parameters}%%%%%%
% Inner parameters
\renewcommand{\SttDimen}{outer}
\renewcommand{\SttDblLineDimen}{middle}
\setlength{\SttBorderWidth}{0pt}
% \renewcommand{\SttBorderColor}{\StateBkgdColor} for record
\FixStateLineDouble{0.6}{0.4}  
%%%%%\section{state line parameters}%%%%%%
\SetStateLineWidth{1.8pt}
\SetStateLineStyle{solid}
\SetStateLineColor{black}
%
\StateLineSimple
%%%%%\section{state label parameters}%%%%%
\RigidStateLabel\FloatingStateLabel\StateLabelInside
\SetStateLabelColor{black}
% \SetStateLabelScale{1.667} (set by the scale picture commands)
\SetStateLabelSize{\normalsize}
\StateLabelModeMath
\SetStateLabelStyle{}
\SetAsideLabelDirct{72}
\SetAsideLabelDistn{6pt}
%%% Variable States
% extra space between the label and the state line (to be fixed)
\setlength{\ExtraSpaceForCrcState}{4mm}
\setlength{\ExtraSpaceForOvlState}{2mm}
\setlength{\ExtraSpaceForRctState}{2mm}
% mode initialisation
\HorizontalStateVarMode\SelfAdjustState
%%% Sizeless States
\setlength{\VerySmallStateDiameter}{.3cm}
%%% Dimmed states
% \renewcommand{\DimStateLineStyle}{solid} 
% \renewcommand{\DimStateLineCoef}{1} % 
% \renewcommand{\DimStateLineColor}{gray}
% \renewcommand{\DimStateLabelColor}{gray}
% \renewcommand{\DimStateBkgdColor}{white}
\SetDimStatePmts{solid}{1}{gray}{gray}{white}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-edges}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge label drawing macros
\renewcommand{\InOutLbl}[2]{#1\!\mid\! #2} % other ex: {(#1, #2)} 
\renewcommand{\IOL}[2]{#1\!\mid\! #2} % downward compatibility 
\renewcommand{\LblCnnct}{+}
%%% Edge drawing parameters
%%% Line
\SetEdgeLineWidth{1pt}			%% width (length param.)
\SetEdgeLineStyle{solid}		%% aspect
\SetEdgeLineColor{black}		%% color
\EdgeLineSimple
% double line the two coefficients have already been initialised in 
% VCSG-edges.tex in order to avoid deadlock; the call to 
% \FixEdgeLineDouble completes the initialisation
\FixEdgeLineDouble{0.5}{0.6}		%% float : coefs*\EdgeLineWidth -> (width of lines, distance)
\SetDblEdgeLineColor{\VCBkgdColor} %% useless since it has 
              %% already been initialised with the picture background
% border
\EdgeLineBorderOff
\FixEdgeLineBorder{2}{\VCBkgdColor}		%% int,color : coef*\EdgeLineWidth -> width of border
%%% Edge arrow
\ArrowEdge				%% fix the style of arrows
% arrows on simple line 
\SetEdgeArrowWidthBase{2.5pt}
\SetEdgeArrowWidthCoef{2}
\SetEdgeArrowLengthCoef{1.4}
\SetEdgeArrowInsetCoef{0.1}
% idem  \SetEdgeArrowDimensions{2pt}{3}{1.4}{0.1}  
% arrows on double line 
\SetDblEdgeArrowWidthBase{2.5pt}
\SetDblEdgeArrowWidthCoef{1.6}
\SetDblEdgeArrowLengthCoef{1.3}
\SetDblEdgeArrowInsetCoef{0.1}
% idem  \SetDblEdgeArrowDimensions{2pt}{3}{1.4}{0.1}  
%%% Edge geometry parameters
\SetEdgeOffset{3pt}
\SetEdgeOffsetCoef{3}
\EdgeOffsetOff
\EdgeOffsetAbs
\SetForthBackEdgeOffsetCoef{2}% coef
\ForthBackOffsetOff
%
\NodeSeparationOff
\SetNodeSep{3pt}
%%% Edge label parameters
\EdgeLabelModeMath
\SetEdgeLabelSize{\normalsize}
\SetEdgeLabelStyle{}
\SetEdgeLabelColor{black}
\SetEdgeLabelScale{1.667}
%%% Edge label boxing parameters
\BoxedEdgeLabelOff
\renewcommand{\BxdEdgLblSep}{5}
\renewcommand{\BxdEdgLblBkg}{white}
\renewcommand{\BxdEdgLblWdt}{1}
\renewcommand{\BxdEdgLblStl}{solid}
\renewcommand{\BxdEdgLblCol}{black}
\renewcommand{\BxdEdgLblDbl}{false}
\renewcommand{\BxdEdgLblRnd}{0}
%%% Edge label geometry parameters
\DirectTransitions
\SetEdgLblPosit{.45}{.55}
\SetArcLblPosit{.4}{.6}
\SetLArcLblPosit{.4}{.6}
\SetLoopLblPosit{.25}{.75}
\SetCLoopLblPosit{.25}{.75}
%
\SetTransLabelSep{8pt}
%
\SwivelEdgeLabel
%%% Dimmed edges
% \renewcommand{\DimEdgeLineStyle}{solid} 
% \renewcommand{\DimEdgeLineCoef}{1.2} 
% \renewcommand{\DimEdgeLineColor}{gray}
% \renewcommand{\DimEdgeLabelColor}{gray}
\SetDimEdgePmts{solid}{1.2}{gray}{gray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Initial-final arrow drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\ArrowOnSmallState}{1.2} 		%float
\renewcommand{\ArrowOnMediumState}{1}		%float : coef *\StateDiameter for size of initial and final arrows
\renewcommand{\ArrowOnLargeState}{.8}		%float
% implicit parameter
\renewcommand{\InitialDir}{w}
\renewcommand{\FinalDir}{e}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Arc geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Angle
\SetArcAngle{15}
\SetLArcAngle{30}
% Curvature
\SetArcCurvature{0.8}
\SetLArcCurvature{0.8}
% Offset
\SetArcOffset{1pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Loop geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Angle
\SetLoopAngle{30}
\SetCLoopAngle{22}
% Preset sizes
\renewcommand{\LoopOnSmallState}{9.6} 		%float
\renewcommand{\LoopOnMediumState}{7}		%float : curvature
\renewcommand{\LoopOnLargeState}{5.8} 		%float
\renewcommand{\CLoopOnSmallState}{12}		%float
\renewcommand{\CLoopOnMediumState}{8}		%float
\renewcommand{\CLoopOnLargeState}{6}		%float
% Offset
\SetLoopOffset{0pt}
%
\MediumStates
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%\section{backward compatibility}%%%%%%
%%%%%  Obsolete commands from version 0.3, 0.4 and 1.0
%%%%%  kept for backward compatibility
%%%%%  cf users manual for description of compatibilty problems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\StateDimen}{outer}
\renewcommand{\StateDblDimen}{middle}
%
\renewcommand{\EdgeLabelPosit}{.45}   
\renewcommand{\EdgeLabelRevPosit}{.55}
\renewcommand{\ArcLabelPosit}{.40}
\renewcommand{\ArcLabelRevPosit}{.60}
\renewcommand{\LArcLabelPosit}{.40}
\renewcommand{\LArcLabelRevPosit}{.60}
\renewcommand{\LoopLabelPosit}{.25}
\renewcommand{\LoopLabelRevPosit}{.75}
\renewcommand{\CLoopLabelPosit}{.25}
\renewcommand{\CLoopLabelRevPosit}{.75}
%
\renewcommand{\LoopVarAngle}{28}
\renewcommand{\LoopOnVariableState}{5.1} 		%float
\renewcommand{\CLoopOnVariableState}{5.2}		%float
\setlength{\LoopVarOffset}{.7pt}
\renewcommand{\LoopOnVerySmallState}{15} 
% label position on initial-final arrow
\renewcommand{\InitStateLabelPosit}{.1}
\renewcommand{\InitStateLabelRevPosit}{.9}
\renewcommand{\FinalStateLabelPosit}{.9}
\renewcommand{\FinalStateLabelRevPosit}{.1}
%
\renewcommand{\ArrowOnVerySmallState}{5} 	%float
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \MediumStates
%%% Shape
%
%%% Variable States
\HorizontalStateVar\SelfAdjustState
%%% Showing -- hiding states
\ShowState
%%% Line
\renewcommand{\VSStateLineCoef}{.6} % coef. for very small state
%%% Background
%%% Label
%%% Label
\setlength{\VertexLineWidth}{0.6pt}             %% length
\renewcommand{\VertexLineColor}{black}        %% color
\renewcommand{\VertexBkgdStyle}{solid} 
\renewcommand{\VertexBkgdColor}{white}        %% color
\SetStateLabelColor{black}		
\renewcommand{\StateLabelScale}{1.7}
\renewcommand{\StateLabelSca}{1}% processing different from other parameters
\RigidLabel\FloatingLabel
%%% Initialisation
\RstState\RstVertex 
%%%%%%%%%%%%%%
%%%%%\section{edge parameters}%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetArcAngle{15}			%% int (degree)
\SetLArcAngle{30}			%% int (degree)
\SetArcCurvature{0.8}			%% float
\SetEdgeOffset{0pt}                     %% length
\SetArcOffset{1pt}			%% length
\SetLoopOffset{0pt}			%% length
\renewcommand{\ForthBackEdgeOffset}{5}	%% float : coef*\EdgeLineWidth -> offset
\FixEdgeBorder{2}{white}		%% int,color : coef*\EdgeLineWidth -> width of border
\FixEdgeLineDouble{0.5}{0.6}		%% float : coefs*\EdgeLineWidth -> (width of lines, distance)
%%%%%%%%%%%%%%
% ZZ aspect
%%%%%%%%%%%%%%
\setlength{\ZZSize}{.9cm}		% length : apparent diameter
\renewcommand{\ZZShape}{0.5}		% coef: opening of the ZZ
\SetZZLineWidth{1.7}			% float
\renewcommand{\TransLabelZZCoef}{0.6}	% float : coef*\ZZSize -> distance added for labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\InitStateLabelPosit}{.10}
\renewcommand{\InitStateLabelRevPosit}{.90}
\renewcommand{\FinalStateLabelPosit}{.90}
\renewcommand{\FinalStateLabelRevPosit}{.10}
% \SetEdgeArrowWidth{5pt}		%length of the edge arrow
% \SetEdgeArrowLengthCoef{1.4}		%float : coef*\EdgeArrowSizeDim width of EA
% \setlength{\EdgeDblArrowWidth}{5.5pt}		%length : size of EA for double transitions
% \renewcommand{\EdgeDblArrowLengthCoef}{1.7}	%int 
% \SetEdgeArrowInsetCoef{0.1}			%float : coef*\EdgeArrowSizeDim
% \SetEdgeArrowStyle{->}				%style (other styles : <-, |-|, -|,...)
% \renewcommand{\EdgeRevArrowStyle}{<-}           %style for reverse transitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initialization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetVCDirectory{}        %default dir=current dir
\HideFrame
\HideGrid
\MediumPicture
\HideName
\RigidLabel
\FullState				%% PlainState
\MediumStates


==> VCPref-slides.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:     VCPref-slides.tex
%%
%% DESCRIPTION:
%%
%%   Contains initial values of VauCanSon-G parameters suitable for 
%%   drawing automata in slides. 
%%   Works with packages `slides', `prosper', or `youpla' for 
%%   instance. A `VCPref-beamer.tex' exists which gives smaller scale 
%%   values. 
%%  
%% DATE:    2008/12/28
%%
%% Copyright (C) 2009 Sylvain Lombardy and Jacques Sakarovitch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scales  --- slides settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\LargeScale}{1.5}
\renewcommand{\MediumScale}{1.16}
\renewcommand{\SmallScale}{0.92}
\renewcommand{\TinyScale}{0.75}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% State aspect
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetStateLineColor{blue}
\SetStateLineWidth{2pt}
\SetStateFillColor{Cyan}
\SetStateLabelColor{Sepia}
\FixDimState{solid}{YellowOrange}{1}{YellowOrange}{white}
%%%%%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetEdgeLineColor{Mahogany}
\SetEdgeLineWidth{1.2pt}
\SetEdgeLabelColor{OliveGreen}
%%% Dimmed edges
\FixDimEdge{dashed}{1.2}{Apricot}{Apricot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput


==> VCPref-version04.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:     VCPref-version04.tex
%%
%% DESCRIPTION:
%%
%%   Set up initial values and default modes and restores function 
%%   behaviours so that total copatibility with version 0.4 is assured.
%%    
%%   Made necessary for the call to \FixedSizeState mode
%%  
%% DATE:    2009/10/28
%%
%% Copyright (C) 2009 Sylvain Lombardy and Jacques Sakarovitch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Default modes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\FixedSizeState
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput


==> VCPref-version1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:     VCPref-version1.tex
%%
%% DESCRIPTION:
%%
%%   Set back to initial values and default modes and restores function 
%%   behaviours of version 1 after a call to  VCPref-version04.
%%    
%%  
%% DATE:    2009/10/28
%%
%% Copyright (C) 2009 Sylvain Lombardy and Jacques Sakarovitch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Default modes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SelfAdjustState
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput


==> VCSG-Preferences.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:    VCSG-Preferences
%%
%% DESCRIPTION:  Initial setting of VauCanSon-G's parameters
%%
%  VCSG-Preferences.tex is required to initialize VauCanSon-G:
%  VauCanSon-G does not perform any initialisation.
%  The values set in this file are mainly those used in EAT
%  
%  The file can also be used as a template to write 
%  a customized style of Vaucanson.
%  
%  VauCanSon-G is cut into 3 main files :
%  VCSG-environment.tex,  VCSG-states.tex,  and VCSG-edges.tex
%  VCSG-Preferences.tex has 3 parts corresponding to each of these 
%  files; inside a part the initialisation follows the appearance of  
%  the parameters in the file
%%  
%% DATE:    2008/12/28
%%
%% Copyright (C) 2009 Sylvain Lombardy and Jacques Sakarovitch
%    2.0 - 041112
%    2.2 - 050727 -- 050818
%    2.3 - 060627; 060717
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-environment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Scaling matters}%%%%%  
% Inner parameters
\renewcommand{\LargeScale}{0.85}    %float : argument of a \scalebox
\renewcommand{\LargeScaleI}{1.18}
\renewcommand{\MediumScale}{0.6}    %float
\renewcommand{\MediumScaleI}{1.67}
\renewcommand{\SmallScale}{0.5}     %float
\renewcommand{\SmallScaleI}{2}
\renewcommand{\TinyScale}{0.42}     %float
\renewcommand{\TinyScaleI}{2.38}
%
\MediumPictures
\FixVCGridScale{1}
%%%%%\section{Picture directory}%%%%%
% \SetVCDirectory{}  % for record : the definition of \VCDirectory is 
%                    % an initialisation 
%%%%%\section{Picture framing}%%%%%
% Inner parameters
\setlength{\VCFrameLineWidth}{0.6pt}
\renewcommand{\VCFrameLineColor}{black}
\setlength{\VCGridLineWidth}{0.6pt}
\renewcommand{\VCGridLineColor}{black}
%
\SetVCBkgdStyle{solid} % Also set StateBkgd, SmallStateBkgd,
                       % SttBorderColor,EdgeLineBorderColor
\SetVCBkgdColor{white} % and DblEdgeLineColor
%
\HideFrame\HideGrid\HideName
%%%%%\section{Picture drawing call}%%%%%
\FixVerticalPlacement{0.5} %float 
%%%%%\section{VauCanSon-G modes}%%%%%
\Automata 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-states}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{node mode}%%%%%%
% \SizedNodes % for record; not necessary after the call to \Automata 
%%%%%\section{state size}%%%%%%
\setlength{\SmallStateDiameter}{.6cm}
\setlength{\MediumStateDiameter}{1cm}
\setlength{\LargeStateDiameter}{1.2cm}
% \FixStateSizes{.6cm}{.9cm}{1.2cm}{.3cm} would have the same effect
%
% \MediumStates postponed after the definition of loop geometry 
% parameters
%%%%%\section{state shape}%%%%%
\CircleStates
\SetOvalStateRatio{\GoldMeanI}
\SetRectangleStateRatio{\GoldMeanI}
%
\SharpStateCorners 
\StateCornerRoundingAbsolute
\SetStateCornerRelRadius{0}
\SetStateCornerRadius{0.2cm}
%%%%%\section{Hiding -- showing}%%%%%
\ShowStates
%%%%%\section{state background parameters}%%%%%
% for record: setting done when setting the Bkgd of the picture 
% \SetStateBkgdStyle{\VCBkgdStyle}\SetStateBkgdColor{\VCBkgdColor}
% \SetSmallStateBkgdStyle{\VCBkgdStyle}
% \SetSmallStateBkgdColor{\VCBkgdColor}
%%%%%\section{construction line parameters}%%%%%%
\renewcommand{\SqrSttCtrClr}{blue}
\renewcommand{\LblBxLnClr}{red}
\renewcommand{\PhtSttLnClr}{green}
\CtrBxLblOff
\CtrSqrSttOff
\CtrPhtSttOff
\setlength{\PhtSttCtr}{0pt} %%% 
%%%%%\section{state line parameters}%%%%%%
% Inner parameters
\renewcommand{\SttDimen}{outer}
\renewcommand{\SttDblLineDimen}{middle}
\setlength{\SttBorderWidth}{0pt}
% \renewcommand{\SttBorderColor}{\StateBkgdColor} for record
\FixStateLineDouble{0.6}{0.4}  
%%%%%\section{state line parameters}%%%%%%
\SetStateLineWidth{1.8pt}
\SetStateLineStyle{solid}
\SetStateLineColor{black}
%
\StateLineSimple
%%%%%\section{state label parameters}%%%%%
\RigidStateLabel\FloatingStateLabel\StateLabelInside
\SetStateLabelColor{black}
% \SetStateLabelScale{1.667} (set by the scale picture commands)
\SetStateLabelSize{\normalsize}
\StateLabelModeMath
\SetStateLabelStyle{}
\SetAsideLabelDirct{72}
\SetAsideLabelDistn{6pt}
%%% Variable States
% extra space between the label and the state line (to be fixed)
\setlength{\ExtraSpaceForCrcState}{4mm}
\setlength{\ExtraSpaceForOvlState}{2mm}
\setlength{\ExtraSpaceForRctState}{2mm}
% mode initialisation
\HorizontalStateVarMode\SelfAdjustState
%%% Sizeless States
\setlength{\VerySmallStateDiameter}{.3cm}
%%% Dimmed states
% \renewcommand{\DimStateLineStyle}{solid} 
% \renewcommand{\DimStateLineCoef}{1} % 
% \renewcommand{\DimStateLineColor}{gray}
% \renewcommand{\DimStateLabelColor}{gray}
% \renewcommand{\DimStateBkgdColor}{white}
\SetDimStatePmts{solid}{1}{gray}{gray}{white}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-edges}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge label drawing macros
\renewcommand{\InOutLbl}[2]{#1\!\mid\! #2} % other ex: {(#1, #2)} 
\renewcommand{\IOL}[2]{#1\!\mid\! #2} % downward compatibility 
\renewcommand{\LblCnnct}{+}
%%% Edge drawing parameters
%%% Line
\SetEdgeLineWidth{1pt}			%% width (length param.)
\SetEdgeLineStyle{solid}		%% aspect
\SetEdgeLineColor{black}		%% color
\EdgeLineSimple
% double line the two coefficients have already been initialised in 
% VCSG-edges.tex in order to avoid deadlock; the call to 
% \FixEdgeLineDouble completes the initialisation
\FixEdgeLineDouble{0.5}{0.6}		%% float : coefs*\EdgeLineWidth -> (width of lines, distance)
\SetDblEdgeLineColor{\VCBkgdColor} %% useless since it has 
              %% already been initialised with the picture background
% border
\EdgeLineBorderOff
\FixEdgeLineBorder{2}{\VCBkgdColor}		%% int,color : coef*\EdgeLineWidth -> width of border
%%% Edge arrow
\ArrowEdge				%% fix the style of arrows
% arrows on simple line 
\SetEdgeArrowWidthBase{2.5pt}
\SetEdgeArrowWidthCoef{2}
\SetEdgeArrowLengthCoef{1.4}
\SetEdgeArrowInsetCoef{0.1}
% idem  \SetEdgeArrowDimensions{2pt}{3}{1.4}{0.1}  
% arrows on double line 
\SetDblEdgeArrowWidthBase{2.5pt}
\SetDblEdgeArrowWidthCoef{1.6}
\SetDblEdgeArrowLengthCoef{1.3}
\SetDblEdgeArrowInsetCoef{0.1}
% idem  \SetDblEdgeArrowDimensions{2pt}{3}{1.4}{0.1}  
%%% Edge geometry parameters
\SetEdgeOffset{3pt}
\SetEdgeOffsetCoef{3}
\EdgeOffsetOff
\EdgeOffsetAbs
\SetForthBackEdgeOffsetCoef{2}% coef
\ForthBackOffsetOff
%
\NodeSeparationOff
\SetNodeSep{3pt}
%%% Edge label parameters
\EdgeLabelModeMath
\SetEdgeLabelSize{\normalsize}
\SetEdgeLabelStyle{}
\SetEdgeLabelColor{black}
\SetEdgeLabelScale{1.667}
%%% Edge label boxing parameters
\BoxedEdgeLabelOff
\renewcommand{\BxdEdgLblSep}{5}
\renewcommand{\BxdEdgLblBkg}{white}
\renewcommand{\BxdEdgLblWdt}{1}
\renewcommand{\BxdEdgLblStl}{solid}
\renewcommand{\BxdEdgLblCol}{black}
\renewcommand{\BxdEdgLblDbl}{false}
\renewcommand{\BxdEdgLblRnd}{0}
%%% Edge label geometry parameters
\DirectTransitions
\SetEdgLblPosit{.45}{.55}
\SetArcLblPosit{.4}{.6}
\SetLArcLblPosit{.4}{.6}
\SetLoopLblPosit{.25}{.75}
\SetCLoopLblPosit{.25}{.75}
%
\SetTransLabelSep{8pt}
%
\SwivelEdgeLabel
%%% Dimmed edges
% \renewcommand{\DimEdgeLineStyle}{solid} 
% \renewcommand{\DimEdgeLineCoef}{1.2} 
% \renewcommand{\DimEdgeLineColor}{gray}
% \renewcommand{\DimEdgeLabelColor}{gray}
\SetDimEdgePmts{solid}{1.2}{gray}{gray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Initial-final arrow drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\ArrowOnSmallState}{1.2} 		%float
\renewcommand{\ArrowOnMediumState}{1}		%float : coef *\StateDiameter for size of initial and final arrows
\renewcommand{\ArrowOnLargeState}{.8}		%float
% implicit parameter
\renewcommand{\InitialDir}{w}
\renewcommand{\FinalDir}{e}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Arc geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Angle
\SetArcAngle{15}
\SetLArcAngle{30}
% Curvature
\SetArcCurvature{0.8}
\SetLArcCurvature{0.8}
% Offset
\SetArcOffset{1pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Loop geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Angle
\SetLoopAngle{30}
\SetCLoopAngle{22}
% Preset sizes
\renewcommand{\LoopOnSmallState}{9.6} 		%float
\renewcommand{\LoopOnMediumState}{7}		%float : curvature
\renewcommand{\LoopOnLargeState}{5.8} 		%float
\renewcommand{\CLoopOnSmallState}{12}		%float
\renewcommand{\CLoopOnMediumState}{8}		%float
\renewcommand{\CLoopOnLargeState}{6}		%float
% Offset
\SetLoopOffset{0pt}
%
\MediumStates
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%\section{backward compatibility}%%%%%%
%%%%%  Obsolete commands from version 0.3, 0.4 and 1.0
%%%%%  kept for backward compatibility
%%%%%  cf users manual for description of compatibilty problems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\StateDimen}{outer}
\renewcommand{\StateDblDimen}{middle}
%
\renewcommand{\EdgeLabelPosit}{.45}   
\renewcommand{\EdgeLabelRevPosit}{.55}
\renewcommand{\ArcLabelPosit}{.40}
\renewcommand{\ArcLabelRevPosit}{.60}
\renewcommand{\LArcLabelPosit}{.40}
\renewcommand{\LArcLabelRevPosit}{.60}
\renewcommand{\LoopLabelPosit}{.25}
\renewcommand{\LoopLabelRevPosit}{.75}
\renewcommand{\CLoopLabelPosit}{.25}
\renewcommand{\CLoopLabelRevPosit}{.75}
%
\renewcommand{\LoopVarAngle}{28}
\renewcommand{\LoopOnVariableState}{5.1} 		%float
\renewcommand{\CLoopOnVariableState}{5.2}		%float
\setlength{\LoopVarOffset}{.7pt}
\renewcommand{\LoopOnVerySmallState}{15} 
% label position on initial-final arrow
\renewcommand{\InitStateLabelPosit}{.1}
\renewcommand{\InitStateLabelRevPosit}{.9}
\renewcommand{\FinalStateLabelPosit}{.9}
\renewcommand{\FinalStateLabelRevPosit}{.1}
%
\renewcommand{\ArrowOnVerySmallState}{5} 	%float
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \MediumStates
%%% Shape
%
%%% Variable States
\HorizontalStateVar\SelfAdjustState
%%% Showing -- hiding states
\ShowState
%%% Line
\renewcommand{\VSStateLineCoef}{.6} % coef. for very small state
%%% Background
%%% Label
%%% Label
\setlength{\VertexLineWidth}{0.6pt}             %% length
\renewcommand{\VertexLineColor}{black}        %% color
\renewcommand{\VertexBkgdStyle}{solid} 
\renewcommand{\VertexBkgdColor}{white}        %% color
\SetStateLabelColor{black}		
\renewcommand{\StateLabelScale}{1.7}
\renewcommand{\StateLabelSca}{1}% processing different from other parameters
\RigidLabel\FloatingLabel
%%% Initialisation
\RstState\RstVertex 
%%%%%%%%%%%%%%
%%%%%\section{edge parameters}%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetArcAngle{15}			%% int (degree)
\SetLArcAngle{30}			%% int (degree)
\SetArcCurvature{0.8}			%% float
\SetEdgeOffset{0pt}                     %% length
\SetArcOffset{1pt}			%% length
\SetLoopOffset{0pt}			%% length
\renewcommand{\ForthBackEdgeOffset}{5}	%% float : coef*\EdgeLineWidth -> offset
\FixEdgeBorder{2}{white}		%% int,color : coef*\EdgeLineWidth -> width of border
\FixEdgeLineDouble{0.5}{0.6}		%% float : coefs*\EdgeLineWidth -> (width of lines, distance)
%%%%%%%%%%%%%%
% ZZ aspect
%%%%%%%%%%%%%%
\setlength{\ZZSize}{.9cm}		% length : apparent diameter
\renewcommand{\ZZShape}{0.5}		% coef: opening of the ZZ
\SetZZLineWidth{1.7}			% float
\renewcommand{\TransLabelZZCoef}{0.6}	% float : coef*\ZZSize -> distance added for labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\InitStateLabelPosit}{.10}
\renewcommand{\InitStateLabelRevPosit}{.90}
\renewcommand{\FinalStateLabelPosit}{.90}
\renewcommand{\FinalStateLabelRevPosit}{.10}
% \SetEdgeArrowWidth{5pt}		%length of the edge arrow
% \SetEdgeArrowLengthCoef{1.4}		%float : coef*\EdgeArrowSizeDim width of EA
% \setlength{\EdgeDblArrowWidth}{5.5pt}		%length : size of EA for double transitions
% \renewcommand{\EdgeDblArrowLengthCoef}{1.7}	%int 
% \SetEdgeArrowInsetCoef{0.1}			%float : coef*\EdgeArrowSizeDim
% \SetEdgeArrowStyle{->}				%style (other styles : <-, |-|, -|,...)
% \renewcommand{\EdgeRevArrowStyle}{<-}           %style for reverse transitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initialization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetVCDirectory{}        %default dir=current dir
\HideFrame
\HideGrid
\MediumPicture
\HideName
\RigidLabel
\FullState				%% PlainState
\MediumStates


==> VCSG-edges.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:    VCSG-edges.tex
%%
%% DESCRIPTION:     Commands for drawing edges
%%
%%   Auxiliary functions and variables called inside VauCanSon-G 
%%   PSTricks commands to be used inside pictures with VauCanSon-G's 
%%   syntax 
%%  
%% DATE:    2008/12/28
%%
%% Copyright (C) 2009 Sylvain Lombardy and Jacques Sakarovitch
%    2.3 - 060627    Copy of the "edge" part of VauCanSon-G 
%                    and adaptation to VCSG-states style
%    081228    transfer of macros from VCSG-functions 
%              transfer of PSTricks function Point to VCSG-functions  
%    091017    modif. EdgeOffset
%              modif. Edge composition label in order to take into 
%                     account \RigidEdgeLabel flag
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{Edge label drawing macros}%%%%%%%%
%%% Layout of compound labels (usage \InOutLbl{input}{output})
% to be initialised in preferences
\newcommand{\InOutLbl}[2]{}
\newcommand{\IOL}[2]{} % downward compatibility 
%%% Connector in lined or stacked labels 
\newcommand{\LblCnnct}{} % to be initialised in preferences
%%% Macros
%%% Stacked labels
\newcommand{\StackTwoLabels}[2]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{@{}c@{}}#1\\ #2 \end{array}%
   \renewcommand{\arraystretch}{1.333}}
\newcommand{\StackThreeLabels}[3]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ #2 \\ #3 \end{array}%
   \renewcommand{\arraystretch}{1.333}}
%%% Stacked labels with \LblCnnct
\newcommand{\StackTwoLabelsP}[2]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ \LblCnnct \\ #2 \end{array}%
   \renewcommand{\arraystretch}{1.333}}
\newcommand{\StackThreeLabelsP}[3]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ \LblCnnct\\#2\\ \LblCnnct\\#3\end{array}% 
   \renewcommand{\arraystretch}{1.333}}
%%% Lined up labels (with \LblCnnct)
\newcommand{\LineTwoLabelsP}[2]{#1 \LblCnnct #2} 
\newcommand{\LineThreeLabelsP}[3]{#1\LblCnnct #2\LblCnnct #3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\VarLoopOn}{\ChgLoopOffset{\LoopVarOff}%
   \ChgLoopSize{\LoopVarSi}%
   \ChgLoopAngle{\LoopVarAng}}
\newcommand{\VarLoopOff}{\RstLoopOffset \RstLoopSize \RstLoopAngle}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \section{Edge parameters}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \subsection{Edge drawing parameters}%%%%%%
%%% \subsubsection{Line}
\newlength{\EdgeLineWidth}\newlength{\EdgeLineWid}
\newcommand{\EdgeLineStyle}{}\newcommand{\EdgeLineSty}{}
\newcommand{\EdgeLineColor}{}\newcommand{\EdgeLineCol}{}
% changing/setting the width of edge line 
\newcommand{\ChgEdgeLineWidth}[1]% coefficient !
   {\setlength{\EdgeLineWid}{#1\EdgeLineWidth}%
    \SetEdgeLineBorderWidth%  %% update the width of border
    \SetDblEdgLineWD%    %% update the width of double line
    \SetEdgArrowWD%      %% see arrow section
    \SetDblEdgArrowWD%   %% see arrow section
    \SetEdgOffset%   %% see transition offset section
   }  
\newcommand{\RstEdgeLineWidth}{\ChgEdgeLineWidth{1}}
\newcommand{\SetEdgeLineWidth}[1]% ATTN the parameter is a length
   {\setlength{\EdgeLineWidth}{#1}\RstEdgeLineWidth}
% relative changing
\newcommand{\ChgRelEdgeLineWidth}[1]% coefficient !
   {\setlength{\EdgeLineWid}{#1\EdgeLineWid}%
    \SetEdgeLineBorderWidth%  %% update the width of border
    \SetDblEdgLineWD%    %% update the width of double line
    \SetEdgArrowWD%      %% see arrow section
    \SetDblEdgArrowWD%   %% see arrow section
    \SetEdgOffset%   %% see transition offset section
   }
% changing/setting the style of edge line 
\newcommand{\ChgEdgeLineStyle}[1]{\renewcommand{\EdgeLineSty}{#1}}  
\newcommand{\RstEdgeLineStyle}{\ChgEdgeLineStyle{\EdgeLineStyle}}
\newcommand{\SetEdgeLineStyle}[1]%
   {\renewcommand{\EdgeLineStyle}{#1}\RstEdgeLineStyle}
% changing/setting the color of edge line
\newcommand{\ChgEdgeLineColor}[1]{\renewcommand{\EdgeLineCol}{#1}}
\newcommand{\RstEdgeLineColor}{\ChgEdgeLineColor{\EdgeLineColor}}
\newcommand{\SetEdgeLineColor}[1]%
   {\renewcommand{\EdgeLineColor}{#1}\RstEdgeLineColor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \subsubsection{Double line} (internal parameters)
% here we depart from the general policy of postponing initialization  
% setting macros for line width parameter call a macro that uses 
% double line coefficients and setting macro for double line 
% paramaters calls line width parameter.
% hence double line parameters are initialized here directly (ie without 
% using setting macros) and initialization is done normaly without 
% noticing the egg and chicken problem.
\newif\ifDblEdgLine
\newcommand{\DblEdgLine}{} 
\newcommand{\DblEdgLineCoef}{0.5} 
\newcommand{\DblEdgLineSep}{0.6} 
\newcommand{\DblEdgLineColor}{} %% Normaly set to picture bckg color
\newlength{\DblEdgLineWD} %% used to store the total width of double  
                          %% lines (see \SetDblEdgLineWD)
% internal function computes the total width of a double line
\newcommand{\SetDblEdgLineWD}% 
   {\setlength{\DblEdgLineWD}{\DblEdgLineCoef\EdgeLineWid}%
    \addtolength{\DblEdgLineWD}{\DblEdgLineCoef\EdgeLineWid}%
    \addtolength{\DblEdgLineWD}{\DblEdgLineSep\EdgeLineWid}}
% changing/setting the edge doubleline status
\newcommand{\EdgeLineDouble}%
   {\DblEdgLinetrue\renewcommand{\DblEdgLine}{true}}
\newcommand{\EdgeLineSimple}%
      {\DblEdgLinefalse\renewcommand{\DblEdgLine}{false}}
% changing/setting the edge doubleline parameters
\newcommand{\FixEdgeLineDouble}[2]%
   {\renewcommand{\DblEdgLineCoef}{#1}%
    \renewcommand{\DblEdgLineSep}{#2}
    \SetDblEdgLineWD\SetDblEdgArrowWD}
\newcommand{\SetDblEdgeLineColor}[1]%
   {\renewcommand{\DblEdgLineColor}{#1}}
\newcommand{\SetDblEdgeLineCoef}[1]%
   {\renewcommand{\DblEdgLineCoef}{#1}%
    \SetDblEdgLineWD\SetDblEdgArrowWD}
\newcommand{\SetDblEdgeLineSep}[1]%
   {\renewcommand{\DblEdgLineSep}{#1}%
    \SetDblEdgLineWD\SetDblEdgArrowWD}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \subsubsection{Border} (internal parameters)
% Border (of prescribed width and color) on both side of the line for 
% giving  the impression that one line passes above another. 
% May be useful when a transition crosses over another one.
\newif\ifEdgeLineBorder
\newlength{\EdgeLineBorderWidth}\newlength{\EdgeLineBorderWD}
\newcommand{\EdgeLineBorderCoef}{2} %% initialization for the same 
                                    %% reason as double line parameter
\newcommand{\EdgeLineBorderColor}{} %% normally same as picture bkgd 
                                    %% (\VCBkgdColor)
%%%%%
% \EdgeLineBorderWidth contains the width of the border if Border is 
% on. Must be updated  when \EdgeLineBorderCoef OR \EdgeLineWid are 
% changed.
% \EdgeLineBorderWD gives the border width to the style:
% 0pt when Border is off, \EdgeLineBorderWidth when Border is on.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  changing/setting macros 
% changing/setting the edge border status
\newcommand{\SetEdgeLineBorderWidth}% internal function  
   {\setlength{\EdgeLineBorderWidth}{\EdgeLineBorderCoef\EdgeLineWid}%
    \ifEdgeLineBorder%
       \setlength{\EdgeLineBorderWD}{\EdgeLineBorderWidth}%
    \fi}
\newcommand{\SetEdgeLineBorderCoef}[1]%
   {\renewcommand{\EdgeLineBorderCoef}{#1}\SetEdgeLineBorderWidth}
\newcommand{\SetEdgeLineBorderColor}[1]%
   {\renewcommand{\EdgeLineBorderColor}{#1}}
\newcommand{\FixEdgeLineBorder}[2]%
   {\SetEdgeLineBorderCoef{#1}%
    \SetEdgeLineBorderColor{#2}}
%
\newcommand{\EdgeLineBorderOn}%
   {\EdgeLineBordertrue%
    \setlength{\EdgeLineBorderWD}{\EdgeLineBorderWidth}}
\newcommand{\EdgeLineBorderOff}%
   {\EdgeLineBorderfalse
    \setlength{\EdgeLineBorderWD}{0pt}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \subsection{Edge arrow parameters}%%%%%%
% arrow style
\newcommand{\EdgeArrowStyle}{}\newcommand{\EdgeArrowSty}{}
\newcommand{\RevEdgArrowStyle}{}
% arrow dimensions
% as for double line parameters, we depart here from the general 
% policy of postponing initialization  
% setting macros for arrows use line width parameter and setting 
% macro for line width updates arrow dimension (width);
% hence arrow width parameters are initialized here directly (ie without
% using setting macros) and initialization is done normaly. 
\newlength{\EdgArrowWidthDim}
\newlength{\EdgArrowWDBase}       %% internal parameter;
\setlength{\EdgArrowWDBase}{2.5pt}  %% has to be set first
\newcommand{\EdgArrowWidthCoef}{2}
\newcommand{\EdgArrowLengthCoef}{}
\newcommand{\EdgArrowInsetCoef}{}
% arrow for double lines (we may want to have arrows on double lines of 
% (slightly) different shape)
\newlength{\DblEdgArrowWidthDim}
\newlength{\DblEdgArrowWDBase}       %% internal parameter;
\setlength{\DblEdgArrowWDBase}{2.5pt}  %% has to be set first
\newcommand{\DblEdgArrowWidthCoef}{1.6}
\newcommand{\DblEdgArrowLengthCoef}{}
\newcommand{\DblEdgArrowInsetCoef}{}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  setting macros 
% computing the arrow width (internal function)
% (must be called at every change of EdgeLineWidth)
% makes it necessary to initialize 
% Arrow coefficients BEFORE line width
\newcommand{\SetEdgArrowWD}% internal function
   {\setlength{\EdgArrowWidthDim}{\EdgArrowWDBase}%
    \addtolength{\EdgArrowWidthDim}{\EdgArrowWidthCoef\EdgeLineWid}}
\newcommand{\SetDblEdgArrowWD}% internal function
   {\setlength{\DblEdgArrowWidthDim}{\DblEdgArrowWDBase}%
    \addtolength{\DblEdgArrowWidthDim}%
                {\DblEdgArrowWidthCoef\DblEdgLineWD}}
% changing/setting arrow style 
\newcommand{\ChgEdgeArrowStyle}[1]{\renewcommand{\EdgeArrowSty}{#1}}
\newcommand{\RstEdgeArrowStyle}{\ChgEdgeArrowStyle{\EdgeArrowStyle}}
\newcommand{\SetEdgArwStyle}[1]%
   {\renewcommand{\EdgeArrowStyle}{#1}\RstEdgeArrowStyle}
%
\newcommand{\PlainEdge}%
   {\SetEdgArwStyle{-}%
    \renewcommand{\RevEdgArrowStyle}{-}}
\newcommand{\ArrowEdge}%
   {\SetEdgArwStyle{->}%
    \renewcommand{\RevEdgArrowStyle}{<-}}
\newcommand{\DblArrowEdge}%
   {\SetEdgArwStyle{->>}%
    \renewcommand{\RevEdgArrowStyle}{<<-}}
% changing/setting arrow dimensions
\newcommand{\SetEdgeArrowWidthBase}[1]% length!!
   {\setlength{\EdgArrowWDBase}{#1}%
    \SetEdgArrowWD}
\newcommand{\SetEdgeArrowWidthCoef}[1]%
   {\renewcommand{\EdgArrowWidthCoef}{#1}%
    \SetEdgArrowWD}
\newcommand{\SetEdgeArrowLengthCoef}[1]%
   {\renewcommand{\EdgArrowLengthCoef}{#1}}
\newcommand{\SetEdgeArrowInsetCoef}[1]%
   {\renewcommand{\EdgArrowInsetCoef}{#1}}
\newcommand{\FixEdgeArrowDimensions}[4]%
      {\SetEdgeArrowWidthBase{#1}%
       \SetEdgeArrowWidthCoef{#2}%
       \SetEdgeArrowLengthCoef{#3}%
       \SetEdgeArrowInsetCoef{#4}}
%
\newcommand{\SetDblEdgeArrowWidthBase}[1]% length!!
   {\setlength{\DblEdgArrowWDBase}{#1}%
    \SetDblEdgArrowWD}
\newcommand{\SetDblEdgeArrowWidthCoef}[1]%
   {\renewcommand{\DblEdgArrowWidthCoef}{#1}%
    \SetDblEdgArrowWD}
\newcommand{\SetDblEdgeArrowLengthCoef}[1]%
   {\renewcommand{\DblEdgArrowLengthCoef}{#1}}
\newcommand{\SetDblEdgeArrowInsetCoef}[1]%
   {\renewcommand{\DblEdgArrowInsetCoef}{#1}}
\newcommand{\SetDblEdgeArrowDimensions}[4]%
      {\SetDblEdgeArrowWidthBase{#1}%
       \SetDblEdgeArrowWidthCoef{#2}%
       \SetDblEdgeArrowLengthCoef{#3}%
       \SetDblEdgeArrowInsetCoef{#4}}
%
\newcommand{\ReverseTransitions}%
   {\ChgEdgeArrowStyle{\RevEdgArrowStyle}%
    \renewcommand{\EdgLblPos}{\EdgLblRevPosit}%
    \renewcommand{\ArcLblPos}{\ArcLblRevPosit}%
    \renewcommand{\LArcLblPos}{\LArcLblRevPosit}%
    \renewcommand{\LoopLblPos}{\LoopLblRevPosit}%
    \renewcommand{\CLoopLblPos}{\CLoopLblRevPosit}%
%     \renewcommand{\InitStateLblPos}{\InitStateLblRevPosit}%
%     \renewcommand{\FinalStateLblPos}{\FinalStateLblRevPosit}%
   }
\newcommand{\DirectTransitions}%
   {\RstEdgeArrowStyle%
    \renewcommand{\EdgLblPos}{\EdgLblPosit}%
    \renewcommand{\ArcLblPos}{\ArcLblPosit}%
    \renewcommand{\LArcLblPos}{\LArcLblPosit}%
    \renewcommand{\LoopLblPos}{\LoopLblPosit}%
    \renewcommand{\CLoopLblPos}{\CLoopLblPosit}%
%     \renewcommand{\InitStateLblPos}{\InitStateLblPosit}%
%     \renewcommand{\FinalStateLblPos}{\FinalStateLblPosit}%
   }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \section{Edge geometry parameters}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \subsubsection{Transition offset} 
% Implemented with a two-step process: on/off and a length. 
% This length is given as a multiple of EdgeLineWidth OR absolutely. 
% Moreover, for convenience AND upward compatilility, can be 
% superseeded by a ForthBackOffset command
\newif\ifEdgeOffset
\newif\ifEdgOffsetRel
\newlength{\EdgeOffset}\newlength{\EdgeOff}%
\newlength{\EdgOff}% buffer between \EdgeOffset and \EdgeOff
\newcommand{\EdgeOffsetCoef}{}% coef
\newcommand{\EdgOffCoef}{}% coef internal
\newcommand{\ForthBackEdgeOffsetCoef}{}% coef
% changing/setting transition offset
\newcommand{\ChgEdgeOffset}[1]%
   {\renewcommand{\EdgOffCoef}{#1}%
    \setlength{\EdgOff}{\EdgOffCoef\EdgeOffset}%
    \ifEdgeOffset\setlength{\EdgeOff}{\EdgOff}\fi%
    }
\newcommand{\RstEdgeOffset}{\ChgEdgeOffset{1}}
\newcommand{\SetEdgeOffset}[1]%
   {\EdgeOffsetAbs%
    \setlength{\EdgeOffset}{#1}\RstEdgeOffset}
\newcommand{\SetEdgeOffsetCoef}[1]%
   {\EdgeOffsetRel%
    \renewcommand{\EdgeOffsetCoef}{#1}%
    \setlength{\EdgeOffset}{\EdgeOffsetCoef\EdgeLineWid}\RstEdgeOffset}
%
\newcommand{\SetEdgOffset}% internal function, called when \EdgeLineWid changes
   {\ifEdgOffsetRel%
    \setlength{\EdgeOffset}{\EdgeOffsetCoef\EdgeLineWid}%
    \setlength{\EdgOff}{\EdgOffCoef\EdgeOffset}%
    \fi%
    \ifEdgeOffset
       \setlength{\EdgeOff}{\EdgOff}%
    \else
       \ifthenelse{\lengthtest{\EdgeOff > 0pt}}%if true \ForthBackOffset
          {\ForthBackOffsetOn}{}%              %is on
    \fi}
%
\newcommand{\EdgeOffsetOn}{\EdgeOffsettrue\setlength{\EdgeOff}{\EdgOff}}
\newcommand{\EdgeOffsetOff}{\EdgeOffsetfalse\setlength{\EdgeOff}{0pt}}
\newcommand{\EdgeOffsetRel}{\EdgOffsetReltrue}
\newcommand{\EdgeOffsetAbs}{\EdgOffsetRelfalse}
%
\newcommand{\SetForthBackEdgeOffsetCoef}[1]% 
   {\renewcommand{\ForthBackEdgeOffsetCoef}{#1}\ForthBackOffsetOn}%
\newcommand{\ForthBackOffsetOn}%
   {\EdgeOffsetOn\EdgeOffsetRel%   
    \SetEdgeOffsetCoef{\ForthBackEdgeOffsetCoef}}
\newcommand{\ForthBackOffsetOff}%
   {\ifEdgeOffset\setlength{\EdgeOff}{\EdgOff}%
    \else\setlength{\EdgeOff}{0pt}%
    \fi
    \EdgeOffsetOff}
%%%% Initialisation ??? 091017
\EdgeOffsetOff
\EdgeOffsetAbs
%%% \subsubsection{Node separation} 
% Distance between the node and the ends of transitions. 
% (not to be mistaken with the (state line) border). 
% Implemented with a two-step process: on/off and a length. 
% This length is given absolutely; would require more care and 
% procedures if it were a fonction of EdgeLineWidth for instance
\newlength{\NodeSep}\newlength{\NodeSP}%
\newlength{\NdSP}% buffer between \NodeSep and \NodeSP
% changing/setting node separation (normal procedure for length)
\newcommand{\ChgNodeSep}[1]%
   {\setlength{\NdSP}{#1\NodeSep}%
    \ifthenelse{\lengthtest{\NodeSP = 0pt}}% plays the role of a flag
       {}{\NodeSeparationOn}} 
\newcommand{\RstNodeSep}{\ChgNodeSep{1}} 
\newcommand{\SetNodeSep}[1]%
   {\setlength{\NodeSep}{#1}\RstNodeSep}
%
\newcommand{\NodeSeparationOn}{\setlength{\NodeSP}{\NdSP}}
\newcommand{\NodeSeparationOff}{\setlength{\NodeSP}{0pt}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \section{Edge label parameters}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \subsection{\LaTeX parameters}
%%% label mode
\newcommand{\EdgLblMode}{} % Internal variable
% setting the label text mode %%% processed differently
\newcommand{\EdgeLabelModeMath}{\renewcommand{\EdgLblMode}{$}}%
\newcommand{\EdgeLabelModeText}{\renewcommand{\EdgLblMode}{}}%
%%% label size
\newcommand{\EdgeLabelSize}{}\newcommand{\EdgeLabelSz}{}
% changing/setting the label size
\newcommand{\ChgEdgeLabelSize}[1]{\renewcommand{\EdgeLabelSz}{#1}}
\newcommand{\RstEdgeLabelSize}{\ChgEdgeLabelSize{\EdgeLabelSize}}
\newcommand{\SetEdgeLabelSize}[1]%
    {\renewcommand{\EdgeLabelSize}{#1}\RstEdgeLabelSize}
%%% label style
\newcommand{\EdgeLabelStyle}{}\newcommand{\EdgeLabelSty}{}
% changing/setting the label style
\newcommand{\ChgEdgeLabelStyle}[1]{\renewcommand{\EdgeLabelSty}{#1}}
\newcommand{\RstEdgeLabelStyle}{\ChgEdgeLabelStyle{\EdgeLabelStyle}}
\newcommand{\SetEdgeLabelStyle}[1]%
    {\renewcommand{\EdgeLabelStyle}{#1}\RstEdgeLabelStyle}
%%% \subsection{graphical parameters}
%%% label colour
\newcommand{\EdgeLabelColor}{}\newcommand{\EdgeLabelCol}{}
% changing/setting the label color
\newcommand{\ChgEdgeLabelColor}[1]{\renewcommand{\EdgeLabelCol}{#1}}
\newcommand{\RstEdgeLabelColor}{\ChgEdgeLabelColor{\EdgeLabelColor}}
\newcommand{\SetEdgeLabelColor}[1]%
    {\renewcommand{\EdgeLabelColor}{#1}\RstEdgeLabelColor}
%%% label scale
\newcommand{\EdgeLabelScale}{}\newcommand{\EdgeLabelSca}{}
% changing/setting the label scale
\newcommand{\ChgEdgeLabelScale}[1]{\renewcommand{\EdgeLabelSca}{#1}}
\newcommand{\RstEdgeLabelScale}{\ChgEdgeLabelScale{1}}
\newcommand{\SetEdgeLabelScale}[1]%
   {\renewcommand{\EdgeLabelScale}{#1}\RstEdgeLabelScale}
%%% \subsection{Boxed label parameters}
\newif\ifVCBoxedEdgeLabel
\newcommand{\BoxedEdgeLabel}{}\newcommand{\BoxedEdgeLbl}{}
\newcommand{\BoxedEdgeLabelOn}{\VCBoxedEdgeLabeltrue}
\newcommand{\BoxedEdgeLabelOff}{\VCBoxedEdgeLabelfalse}
%
\newcommand{\BxdEdgLblSep}{}
\newcommand{\BxdEdgLblBkg}{}
\newcommand{\BxdEdgLblWdt}{}
\newcommand{\BxdEdgLblStl}{}
\newcommand{\BxdEdgLblCol}{}
\newcommand{\BxdEdgLblDbl}{}
\newcommand{\BxdEdgLblRnd}{}
%%% \subsection{geometric parameters}
%%% position on transitions
\newcommand{\EdgLblPosit}{}\newcommand{\EdgLblRevPosit}{}
\newcommand{\ArcLblPosit}{}\newcommand{\ArcLblRevPosit}{}
\newcommand{\LArcLblPosit}{}\newcommand{\LArcLblRevPosit}{}
\newcommand{\LoopLblPosit}{}\newcommand{\LoopLblRevPosit}{}
\newcommand{\CLoopLblPosit}{}\newcommand{\CLoopLblRevPosit}{}
\newcommand{\EdgLblPos}{}
\newcommand{\ArcLblPos}{}
\newcommand{\LArcLblPos}{}
\newcommand{\LoopLblPos}{}
\newcommand{\CLoopLblPos}{}
% changing/setting position on transitions ???
% \newcommand{\ChgEdgLblPosit}[1]{\renewcommand{\EdgLblPos}{#1}}  
% \newcommand{\RstEdgLblPosit}{\ChgEdgLblPosit{\EdgLblPosit}}
\newcommand{\SetEdgLblPosit}[2]%
   {\renewcommand{\EdgLblPosit}{#1}\renewcommand{\EdgLblPos}{#1}%
    \renewcommand{\EdgLblRevPosit}{#2}}
\newcommand{\SetArcLblPosit}[2]%
   {\renewcommand{\ArcLblPosit}{#1}\renewcommand{\ArcLblPos}{#1}%
    \renewcommand{\ArcLblRevPosit}{#2}}
\newcommand{\SetLArcLblPosit}[2]%
   {\renewcommand{\LArcLblPosit}{#1}\renewcommand{\LArcLblPos}{#1}%
    \renewcommand{\LArcLblRevPosit}{#2}}
\newcommand{\SetLoopLblPosit}[2]%
   {\renewcommand{\LoopLblPosit}{#1}\renewcommand{\LoopLblPos}{#1}%
    \renewcommand{\LoopLblRevPosit}{#2}}
\newcommand{\SetCLoopLblPosit}[2]%
   {\renewcommand{\CLoopLblPosit}{#1}\renewcommand{\CLoopLblPos}{#1}%
    \renewcommand{\CLoopLblRevPosit}{#2}}
%%% distance from transition
\newlength{\TransLabelSep}\newlength{\TransLabelSP}
% changing/setting distance from transition
\newcommand{\ChgTransLabelSep}[1]% coefficient !
   {\setlength{\TransLabelSP}{#1\TransLabelSep}}
\newcommand{\RstTransLabelSep}{\ChgTransLabelSep{1}}
\newcommand{\SetTransLabelSep}[1]% length !
   {\setlength{\TransLabelSep}{#1}\RstTransLabelSep}
\newcommand{\ChgRelTransLabelSep}[1]% coefficient !
      {\setlength{\TransLabelSP}{#1\TransLabelSP}}
%%% orientation
\newif\ifVCRigidEdgeLabel
\newcommand{\RigidEdgeLabel}{\VCRigidEdgeLabeltrue}
\newcommand{\SwivelEdgeLabel}{\VCRigidEdgeLabelfalse}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{dimmed edges}%%%%
%%%  Dimmed edges (e.g. for transitions to non accessible states)
\newcommand{\DimEdgeLineStyle}{} 
\newcommand{\DimEdgeLineCoef}{} 
\newcommand{\DimEdgeLineColor}{}
\newcommand{\DimEdgeLabelColor}{}
%%% establishing the dimmed style
\newcommand{\DimEdge}%
   {\ChgEdgeLineStyle{\DimEdgeLineStyle}%
    \ChgEdgeLineWidth{\DimEdgeLineCoef}%
    \ChgEdgeLineColor{\DimEdgeLineColor}%
    \ChgEdgeLabelColor{\DimEdgeLabelColor}}%
\newcommand{\SetDimEdgePmts}[4]%
   {\renewcommand{\DimEdgeLineStyle}{#1}%
    \renewcommand{\DimEdgeLineCoef}{#2}%
    \renewcommand{\DimEdgeLineColor}{#3}%
    \renewcommand{\DimEdgeLabelColor}{#4}
    \renewcommand{\DimEdge}%
      {\ChgEdgeLineStyle{\DimEdgeLineStyle}%
       \ChgEdgeLineWidth{\DimEdgeLineCoef}%
       \ChgEdgeLineColor{\DimEdgeLineColor}%
       \ChgEdgeLabelColor{\DimEdgeLabelColor}}%
    }%
\newcommand{\UnDimEdge}%
   {\RstEdgeLineStyle%
    \RstEdgeLineWidth%
    \RstEdgeLineColor%
    \RstEdgeLabelColor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% \section{Transition styles}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpsstyle{VCEdgeStyle}%
    {%
     linewidth=\EdgeLineWid,%
     linestyle=\EdgeLineSty,%
     linecolor=\EdgeLineCol,%
     bordercolor=\EdgeLineBorderColor,%
     border=\EdgeLineBorderWD,%
     fillstyle=none,% ???
     doubleline=false,%
%
     arrows=\EdgeArrowSty,%
     arrowsize=\EdgArrowWidthDim,%
     arrowlength=\EdgArrowLengthCoef,%
     arrowinset=\EdgArrowInsetCoef,%
%
     offset=\EdgeOff,%
     labelsep=\TransLabelSP,%
     nodesep=\NodeSP}%
\newpsstyle{VCDblEdgeStyle}% 
    {doubleline=true,%
     linewidth=\DblEdgLineCoef\EdgeLineWid,%
     doublesep=\DblEdgLineSep\EdgeLineWid,%
     doublecolor=\DblEdgLineColor,%
%
     arrowsize=\DblEdgArrowWidthDim,%
     arrowlength=\DblEdgArrowLengthCoef,%
     arrowinset=\DblEdgArrowInsetCoef}
%
\newpsstyle{VCBoxedEdgeLblStyle}%
    {%
     framesep=\BxdEdgLblSep pt,%
     fillstyle=solid,%
     fillcolor=\BxdEdgLblBkg,% 
     linewidth=\BxdEdgLblWdt pt,%
     linestyle=\BxdEdgLblStl,%
     linecolor=\BxdEdgLblCol,%
%      doubleline=\BxdEdgLblDbl,%
     cornersize=relative,%
     framearc=\BxdEdgLblRnd}
%%%
\newcommand{\EdgeStyle}%
   {\psset{style=VCEdgeStyle}%
    \ifDblEdgLine\psset{style=VCDblEdgeStyle}\fi}
\newcommand{\BoxedEdgeLabelStyle}%
   {\psset{style=VCBoxedEdgeLblStyle}}
%%%%%\section{Edge label composition}%%%%%

% \makeatletter
% 
% \def\psRot#1(#2,#3){\***@makebox{\***@Rot#1(#2,#3)}}
% \def\***@Rot#1(#2,#3){%
% \pssetxlength\***@dima{#2}%
% \pssetylength\***@dimb{#3}%
% \leavevmode
% \***@Verb{%
% /xRot \***@number\***@dima\space def
% /yRot \***@number\***@dimb\space def}%
% \hbox{%
% \***@Verb{%
% /cosA #1 cos def
% /sinA #1 sin def
% /ax cosA def
% /by sinA def
% /cx sinA neg def
% /dy cosA def
% /ex xRot cosA mul neg xRot add yRot sinA mul add def
% /fy xRot sinA mul neg yRot add yRot cosA mul sub def
% {[ax by cx dy ex fy] concat
% } \***@TMChange}%
% \box\***@hbox%
% \***@Verb{\***@TMRestore}}}
% 
% \makeatother

\newcommand{\ComposedEdgLbl}[1]%
   {\textcolor{\EdgeLabelCol}%    
      {\scalebox{\EdgeLabelSca}%
         {\scalebox{\EdgeLabelScale}%
            {\EdgeLabelSz 
             \EdgLblMode\EdgeLabelSty{\VCLbl{#1}}\EdgLblMode}}}}%

\newcommand{\VCEdgeLabel}[1]%
    {\ifVCRigidEdgeLabel%
        {\textcolor{\EdgeLabelCol}%
           {\scalebox{\EdgeLabelSca}%
              {\scalebox{\EdgeLabelScale}%
                 {%
%                   \qdisk(0,0){2pt}
                 \Put*[rot={0*}](0,0)%
                    {\EdgeLabelSz%
                     \EdgLblMode\EdgeLabelSty{\VCLbl{#1}}\EdgLblMode}}}}}%
     \else% 
        {\textcolor{\EdgeLabelCol}%
           {\scalebox{\EdgeLabelSca}%
              {\scalebox{\EdgeLabelScale}%
                 {%
%                  \rput{0}(0,0)%
%                 \qdisk(0,0){2pt}%
                    {\EdgeLabelSz%
                     \EdgLblMode\EdgeLabelSty{\VCLbl{#1}}\EdgLblMode}}}}}%
     \fi}%

\newcommand{\naputnrotParam}{\ifVCRigidEdgeLabel N\else 0\fi}
% \newcommand{\mynrot}{\makeatletter\psk@rot\makeatother}
\newcommand{\WRLLbl}[2]%
    {\ifVCBoxedEdgeLabel%
        \BoxedEdgeLabelStyle
        \naput[npos=#1]{\psframebox{\VCEdgeLabel{#2}}}%
     \else%
        \naput*[npos=#1,ref=t,nrot=\naputnrotParam]{\VCEdgeLabel{#2}}%
     \fi}%
\newcommand{\WRRLbl}[2]%
    {\ifVCBoxedEdgeLabel%
        \BoxedEdgeLabelStyle
        \nbput[npos=#1]{\psframebox{\VCEdgeLabel{#2}}}%
     \else%
        \nbput*[npos=#1,ref=ur,nrot=\naputnrotParam]{\VCEdgeLabel{#2}}%
     \fi}%
\newcommand{\WRCLbl}[2]%
    {\ifVCBoxedEdgeLabel%
        \BoxedEdgeLabelStyle
        \ncput[npos=#1]{\psframebox{\VCEdgeLabel{#2}}}%
     \else%
        \ncput[npos=#1,nrot=\naputnrotParam]{\VCEdgeLabel{#2}}%
     \fi}%
% \newcommand{\WRLLbl}[2]%
%     {%
%      \ifVCRigidEdgeLabel%
%      \else%
%         \ifVCBoxedEdgeLabel%
% 	   \BoxedEdgeLabelStyle
% 	   \naput[npos=#1]{\psframebox{\ComposedEdgLbl{#2}}}%
% 	\else%
% 	   \naput[npos=#1]{\ComposedEdgLbl{#2}}%
% 	\fi%
%      \fi}
% \newcommand{\WRRLbl}[2]%
%     {%
%      \ifVCRigidEdgeLabel%
%      \else%
%         \ifVCBoxedEdgeLabel%
%            \BoxedEdgeLabelStyle
% 	   \nbput[npos=#1]{\psframebox{\ComposedEdgLbl{#2}}}%
% 	\else%
% 	   \nbput[npos=#1]{\ComposedEdgLbl{#2}}%
% 	\fi%
%      \fi}
% \newcommand{\WRCLbl}[2]%
%     {%
%      \ifVCRigidEdgeLabel%
%      \else%
%         \ifVCBoxedEdgeLabel%
% 	   \BoxedEdgeLabelStyle
% 	   \ncput[npos=#1]{\psframebox{\ComposedEdgLbl{#2}}}%
% 	\else%
% 	   \ncput[npos=#1]{\ComposedEdgLbl{#2}}%
% 	\fi%
%      \fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  \section{Edge drawing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EdgeL}[4][{\EdgLblPos}]% 
   {\EdgeStyle\ncline{#2}{#3}\WRLLbl{#1}{#4}}
\newcommand{\EdgeR}[4][{\EdgLblPos}]%
   {\EdgeStyle \ncline{#2}{#3}\WRRLbl{#1}{#4}}
\newcommand{\EdgeC}[4][{\EdgLblPos}]%
   {\EdgeStyle \ncline{#2}{#3}\WRCLbl{#1}{#4}}
\newcommand{\Edge}[2]{\EdgeStyle \ncline{#1}{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% line
% label
% \newcommand{\EdgeLabelColor}{black}
% \newcommand{\EdgeLabelScale}{1.7}
% %%% Dimmed edges 
% \newcommand{\DimEdgeLineCoef}{1.2} 
% \newcommand{\DimEdgeLineStyle}{solid} 
% \newcommand{\DimEdgeLineColor}{gray}
% \newcommand{\DimEdgeLabelColor}{gray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  \section{Zigzag edges}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Zigzag edges parameter
\newlength{\ZZSize}
\setlength{\ZZSize}{.9cm}%\MediumStateDiameter
\newcommand{\ZZShape}{0.5}
\newcommand{\ZZLineWidth}{1.7}% coefficient multiplicateur
\newcommand{\TransLabelZZCoef}{0.6}% coefficient multiplicateur
\newlength{\ZZSiZ}
\setlength{\ZZSiZ}{\ZZSize}%
\newcommand{\ZZLineWid}{\ZZLineWidth}% coefficient multiplicateur
% \newcommand{\ZZLineWid}{\ZZLineWidth}% coefficient multiplicateur
%
%%% zig-zag style
\newpsstyle{VCZZStyle}%
    {linewidth=\ZZLineWid\EdgeLineWid,%
     linearc=1.6pt,%
     coilwidth=1.2\ZZSiZ,%
     coilheight=\ZZShape,%
     coilarmA=0.1\ZZSiZ,%
     coilarmB=0.3\ZZSiZ,%
     labelsep=\TransLabelSP}
\newcommand{\ZZStyle}%
   {\addtolength{\TransLabelSP}{\TransLabelZZCoef\ZZSiZ}%
    \psset{style=VCZZStyle}%
    \addtolength{\TransLabelSP}{-\TransLabelZZCoef\ZZSiZ}}
%%% Zigzag edges
\newcommand{\ZZEdge}[2]%
   {\EdgeStyle\ZZStyle\nczigzag{#1}{#2}}
\newcommand{\ZZEdgeL}[4][{\EdgLblPos}]%
   {\EdgeStyle\ZZStyle\nczigzag{#2}{#3}\WRLLbl{#1}{#4}}
\newcommand{\ZZEdgeR}[4][{\EdgLblPos}]%
   {\EdgeStyle\ZZStyle\nczigzag{#2}{#3}\WRRLbl{#1}{#4}}
\newcommand{\ZZEdgeC}[4][{\EdgLblPos}]%
   {\EdgeStyle\ZZStyle\nczigzag{#2}{#3}\WRCLbl{#1}{#4}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge geometric parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Edge label parameters --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% flags 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge geometric parameters  --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Edge label parameters --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% label distance from transition
% \newlength{\TransLabelSP}\setlength{\TransLabelSP}{\TransLabelSep}
% label position on transitions
% \newcommand{\EdgeLabelPos}{\EdgeLabelPosit}
% \newcommand{\ArcLabelPos}{\ArcLabelPosit}
% \newcommand{\LArcLabelPos}{\LArcLabelPosit}
% \newcommand{\LoopLabelPos}{\LoopLabelPosit}
% \newcommand{\CLoopLabelPos}{\CLoopLabelPosit}
% label position on initial-final arrow
\newcommand{\InitStateLabelPos}{\InitStateLabelPosit}
\newcommand{\FinalStateLabelPos}{\FinalStateLabelPosit}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Transition styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%
% \newcommand{\ChgZZSize}[1]{\setlength{\ZZSiZ}{#1}}
% \newcommand{\RstZZSize}{\setlength{\ZZSiZ}{\ZZSize}}
% \newcommand{\SetZZSize}[1]{\setlength{\ZZSiZe}{#1}\RstZZSize}
% %%%\ZZLineWidth
% \newcommand{\ChgZZLineWidth}[1]{\renewcommand{\ZZLineWid}{#1}}
% \newcommand{\RstZZLineWidth}{\ChgZZLineWidth{\ZZLineWidth}}
% \newcommand{\SetZZLineWidth}[1]%
%    {\renewcommand{\ZZLineWidth}{#1}\RstZZLineWidth}
% %
%%% label of transitions
\newcommand{\VaucEdgeLabel}[1]{%
        \textcolor{\EdgeLabelCol}{\scalebox{\EdgeLabelSca}{\scalebox{\EdgeLabelScale}{$ #1 $}}}}
%%%
\newcommand{\RstEdge}{%
   \RstEdgeOffset\RstArcAngle\RstLArcAngle%
   \RstArcCurvature\RstLArcCurvature%
   \RstArcOffset\RstLoopOffset\RstLoopSize%
   \RstEdgeLineColor\RstEdgeLineStyle\RstEdgeLineWidth\EdgeLineSimple%
   \StraightArrow%\EdgeBorderOff%
   \RstEdgeLabelScale\RstEdgeLabelColor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Initial-final arrow drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% implicit parameter
\newcommand{\InitialDir}{}\newcommand{\FinalDir}{}
\newcommand{\Dirnum}{}
%%% Size of initial and final arrow
% the size is relative to the diameter
% and the coefficient varies with the diameter
\newcommand{\ArrowOnStateCoef}{}
\newcommand{\ArrowOnMediumState}{}
\newcommand{\ArrowOnSmallState}{} 
\newcommand{\ArrowOnLargeState}{}
% ??? 120514
\newlength{\IFArwLgt}%
\newcommand{\SetIFArwLgt}{\setlength{\IFArwLgt}{\ArrowOnStateCoef\StateDia}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% compute the distance for initial and final arrows
\newlength{\IFSDst}%
\newcommand{\CptIFSDst}%
   {%
    \setlength{\IFArwLgt}{\ArrowOnStateCoef\StateDia}%
    \VCSGGreaterLgt{\LastSttDrawnWidth}{\LastSttDrawnHeight}{\VCSGTmpLength}%
    \CorrPosSttIntDim{\VCSGTmpLength}%
    \setlength{\IFSDst}{.5\VCSGTmpLength}%
    \addtolength{\IFSDst}{\IFArwLgt}%
    }
% set the end point of initial and final arrows
\newcommand{\SetIFSNode}[2]%
   {%
    \VCSGCompassDecode{#1}{\Dirnum}%
    \CptIFSDst%
    \SpecialCoor%
    \uput{\IFSDst}[\Dirnum](#2){\pnode{#2qif}}%
    \NormalCoor%
    }
% without label new version 1205014
\newcommand{\Initial}[2][\InitialDir]%
   {\SetIFSNode{#1}{#2}%
    \EdgeStyle\ncline{#2qif}{#2}}
\newcommand{\Final}[2][\FinalDir]%
   {\SetIFSNode{#1}{#2}%
    \EdgeStyle\ncline{#2}{#2qif}}
% with label new version 1205014
%  NB modified syntax eg \InitialL[pos]{dir}{statename}{label}
\newcommand{\InitialL}[4][{\InitStateLabelPos}]%
   {\SetIFSNode{#2}{#3}%
    \EdgeStyle\ncline{#3qif}{#3}\naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\InitialR}[4][{\InitStateLabelPos}]%
   {\SetIFSNode{#2}{#3}%
    \EdgeStyle\ncline{#3qif}{#3}\nbput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\FinalL}[4][{\FinalStateLabelPos}]%
   {\SetIFSNode{#2}{#3}%
    \EdgeStyle\ncline{#3}{#3qif}\naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\FinalR}[4][{\FinalStateLabelPos}]%
   {\SetIFSNode{#2}{#3}%
    \EdgeStyle\ncline{#3}{#3qif}\nbput[npos=#1]{\VaucEdgeLabel{#4}}}
% % without label old version
% \newcommand{\Initial}[2][\InitialDir]%
%    {\VCSGCompassDecode{#1}{\Dirnum}%
%     \CptIFSDst%
%     \SpecialCoor%
%     \uput{\IFSDst}[\Dirnum](#2){\pnode{qz}}%
%     \NormalCoor%
%     \EdgeStyle\ncline{qz}{#2}}
% \newcommand{\Final}[2][\FinalDir]%
%    {\VCSGCompassDecode{#1}{\Dirnum}%
%     \CptIFSDst%
%     \SpecialCoor%
%     \uput{\IFSDst}[\Dirnum](#2){\pnode{qz}}%
%     \NormalCoor%
%     \EdgeStyle\ncline{#2}{qz}}
% % with label
% %  NB modified syntax eg \InitialL[pos]{dir}{statename}{label}
% \newcommand{\InitialL}[4][{\InitStateLabelPos}]%
%    {\EdgeStyle\ncline{#3#2}{#3}\naput[npos=#1]{\VaucEdgeLabel{#4}}}
% \newcommand{\InitialR}[4][{\InitStateLabelPos}]%
%    {\EdgeStyle\ncline{#3#2}{#3}\nbput[npos=#1]{\VaucEdgeLabel{#4}}}
% \newcommand{\FinalL}[4][{\FinalStateLabelPos}]%
%    {\EdgeStyle\ncline{#3}{#3#2}\naput[npos=#1]{\VaucEdgeLabel{#4}}}
% \newcommand{\FinalR}[4][{\FinalStateLabelPos}]%
%    {\EdgeStyle\ncline{#3}{#3#2}\nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Arc drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Arc parameters
% Angle
\newcommand{\ArcAngle}{}\newcommand{\ArcAng}{}
\newcommand{\LArcAngle}{}\newcommand{\LArcAng}{}
% Curvature
\newcommand{\ArcCurvature}{}\newcommand{\ArcCurv}{}
\newcommand{\LArcCurvature}{}\newcommand{\LArcCurv}{}
% Offset
\newlength{\ArcOffset}\newlength{\ArcOff}
%%% Arc parameter changing/setting
\newcommand{\ChgArcAngle}[1]{\renewcommand{\ArcAng}{#1}}
\newcommand{\RstArcAngle}{\ChgArcAngle{\ArcAngle}}
\newcommand{\SetArcAngle}[1]%
   {\renewcommand{\ArcAngle}{#1}\RstArcAngle}
%
\newcommand{\ChgLArcAngle}[1]{\renewcommand{\LArcAng}{#1}}
\newcommand{\RstLArcAngle}{\ChgLArcAngle{\LArcAngle}}
\newcommand{\SetLArcAngle}[1]%
   {\renewcommand{\LArcAngle}{#1}\RstLArcAngle}
%
\newcommand{\ChgArcCurvature}[1]{\renewcommand{\ArcCurv}{#1}}
\newcommand{\RstArcCurvature}{\ChgArcCurvature{\ArcCurvature}}
\newcommand{\SetArcCurvature}[1]%
   {\renewcommand{\ArcCurvature}{#1}\RstArcCurvature}
%
\newcommand{\ChgLArcCurvature}[1]{\renewcommand{\LArcCurv}{#1}}
\newcommand{\RstLArcCurvature}{\ChgLArcCurvature{\LArcCurvature}}
\newcommand{\SetLArcCurvature}[1]%
   {\renewcommand{\LArcCurvature}{#1}\RstLArcCurvature}
%
\newcommand{\ChgArcOffset}[1]{\setlength{\ArcOff}{#1}}
\newcommand{\RstArcOffset}{\setlength{\ArcOff}{\ArcOffset}}
\newcommand{\SetArcOffset}[1]%
   {\renewcommand{\ArcOffset}{#1}\RstArcOffset}
%%% Arc drawing styles
\newcommand{\ArcLStyle}%
    {\psset{ncurv=\ArcCurv,arcangle=\ArcAng,offset=\ArcOff}}
\newcommand{\ArcRStyle}%
    {\psset{ncurv=\ArcCurv,arcangle=-\ArcAng,offset=-\ArcOff}}
\newcommand{\LArcLStyle}%
    {\psset{ncurv=\LArcCurv,arcangle=\LArcAng,offset=\ArcOff}}
\newcommand{\LArcRStyle}%
    {\psset{ncurv=\LArcCurv,arcangle=-\LArcAng,offset=-\ArcOff}}
%%% Arc drawing commands
\newcommand{\ArcL}[4][{\ArcLblPos}]%
   {\EdgeStyle \ArcLStyle \ncarc{#2}{#3} \WRLLbl{#1}{#4}}%\naput[npos=#1]{\VCEdgeLabel{#4}}
\newcommand{\ArcR}[4][{\ArcLblPos}]%
   {\EdgeStyle \ArcRStyle \ncarc{#2}{#3} \WRRLbl{#1}{#4}}%
\newcommand{\LArcL}[4][{\LArcLblPos}]%
   {\EdgeStyle \LArcLStyle \ncarc{#2}{#3} \WRLLbl{#1}{#4}}%
\newcommand{\LArcR}[4][{\LArcLblPos}]%
   {\EdgeStyle \LArcRStyle \ncarc{#2}{#3} \WRRLbl{#1}{#4}}%
\newcommand{\ArcLC}[4][{\ArcLblPos}]%
   {\EdgeStyle \ArcLStyle \ncarc{#2}{#3} \WRCLbl{#1}{#4}}%\naput[npos=#1]{\VCEdgeLabel{#4}}
\newcommand{\ArcRC}[4][{\ArcLblPos}]%
   {\EdgeStyle \ArcRStyle \ncarc{#2}{#3} \WRCLbl{#1}{#4}}%
\newcommand{\LArcLC}[4][{\LArcLblPos}]%
   {\EdgeStyle \LArcLStyle \ncarc{#2}{#3} \WRCLbl{#1}{#4}}%
\newcommand{\LArcRC}[4][{\LArcLblPos}]%
   {\EdgeStyle \LArcRStyle \ncarc{#2}{#3} \WRCLbl{#1}{#4}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Loop drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Loop parameters
% Angle
\newcommand{\LoopAngle}{}\newcommand{\LoopAng}{}
\newcommand{\CLoopAngle}{}\newcommand{\CLoopAng}{}
% Size
\newcommand{\LoopSize}{}\newcommand{\LoopSi}{}
\newcommand{\CLoopSize}{}\newcommand{\CLoopSi}{}
% Offset
\newlength{\LoopOffset}\newlength{\LoopOff}
% Preset sizes of loops (depending on the size of the state)
\newcommand{\LoopOnSmallState}{} 
\newcommand{\LoopOnMediumState}{}
\newcommand{\LoopOnLargeState}{} 
%
\newcommand{\CLoopOnSmallState}{}
\newcommand{\CLoopOnMediumState}{}
\newcommand{\CLoopOnLargeState}{}
%%% Loop parameters% Size
%
\newcommand{\ChgLoopSize}[1]{\renewcommand{\LoopSi}{#1}}
\newcommand{\RstLoopSize}{\ChgLoopSize{\LoopSize}}
\newcommand{\SetLoopSize}[1]%
   {\renewcommand{\LoopSize}{#1}\RstLoopSize}
%
\newcommand{\ChgCLoopSize}[1]{\renewcommand{\CLoopSi}{#1}}
\newcommand{\RstCLoopSize}{\ChgCLoopSize{\CLoopSize}}
\newcommand{\SetCLoopSize}[1]%
   {\renewcommand{\CLoopSize}{#1}\RstCLoopSize}
% Angle
\newcommand{\ChgLoopAngle}[1]{\renewcommand{\LoopAng}{#1}}
\newcommand{\RstLoopAngle}{\ChgLoopAngle{\LoopAngle}}
\newcommand{\SetLoopAngle}[1]%
   {\renewcommand{\LoopAngle}{#1}\RstLoopAngle}
%
\newcommand{\ChgCLoopAngle}[1]{\renewcommand{\CLoopAng}{#1}}
\newcommand{\RstCLoopAngle}{\ChgCLoopAngle{\CLoopAngle}}
\newcommand{\SetCLoopAngle}[1]%
   {\renewcommand{\CLoopAngle}{#1}\RstCLoopAngle}
% Offset
\newcommand{\ChgLoopOffset}[1]{\setlength{\LoopOff}{#1}}
\newcommand{\RstLoopOffset}{\setlength{\LoopOff}{\LoopOffset}}
\newcommand{\SetLoopOffset}[1]%
   {\renewcommand{\LoopOffset}{#1}\RstLoopOffset}
%
%%%%
\newcounter{anglea}\newcounter{angleb}
\newcommand{\LoopXR}[7]%
   {{\setcounter{anglea}{#2-#4}}%
    {\setcounter{angleb}{#2+#4}}%
    {\EdgeStyle \psset{angleA=\theanglea,angleB=\theangleb,offset=#5,ncurv=#6}% 
    \nccurve{#3}{#3} \WRRLbl{#1}{#7}}}%\nbput[npos=#1]{\VaucEdgeLabel{#7}}
\newcommand{\LoopXL}[7]%
   {{\setcounter{anglea}{#2+#4}}%
    {\setcounter{angleb}{#2-#4}}%
    {\EdgeStyle \psset{angleA=\theanglea,angleB=\theangleb,offset=-#5,ncurv=#6}% 
    \nccurve{#3}{#3} \WRLLbl{#1}{#7}}}%\naput[npos=#1]{\VaucEdgeLabel{#7}}
\newcommand{\LoopR}[4][{\LoopLblPos}]%
   {\LoopXR{#1}{#2}{#3}{\LoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\LoopL}[4][{\LoopLblPos}]%
   {\LoopXL{#1}{#2}{#3}{\LoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\CLoopR}[4][{\CLoopLblPos}]%
   {\LoopXR{#1}{#2}{#3}{\CLoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\CLoopL}[4][{\CLoopLblPos}]%
   {\LoopXL{#1}{#2}{#3}{\CLoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\LoopVarR}[4][{\LoopLblPos}]%
   {\LoopXR{#1}{#2}{#3}{\LoopVarAng}{\LoopVarOff}{\LoopVarSi}{#4}}
\newcommand{\LoopVarL}[4][{\LoopLblPos}]%
   {\LoopXL{#1}{#2}{#3}{\LoopVarAng}{\LoopVarOff}{\LoopVarSi}{#4}}
\newcommand{\LoopW}[3][{\LoopLblPos}]{\LoopR[#1]{180}{#2}{#3}}
\newcommand{\LoopE}[3][{\LoopLblPos}]{\LoopL[#1]{0}{#2}{#3}}
\newcommand{\LoopN}[3][{\LoopLblPos}]{\LoopL[#1]{90}{#2}{#3}}
\newcommand{\LoopS}[3][{\LoopLblPos}]{\LoopR[#1]{-90}{#2}{#3}}
\newcommand{\LoopNW}[3][{\LoopLblPos}]{\LoopR[#1]{135}{#2}{#3}}
\newcommand{\LoopNE}[3][{\LoopLblPos}]{\LoopL[#1]{45}{#2}{#3}}
\newcommand{\LoopSW}[3][{\LoopLblPos}]{\LoopL[#1]{-135}{#2}{#3}}
\newcommand{\LoopSE}[3][{\LoopLblPos}]{\LoopR[#1]{-45}{#2}{#3}}
\newcommand{\CLoopW}[3][{\CLoopLblPos}]{\CLoopR[#1]{180}{#2}{#3}}
\newcommand{\CLoopE}[3][{\CLoopLblPos}]{\CLoopL[#1]{0}{#2}{#3}}
\newcommand{\CLoopN}[3][{\CLoopLblPos}]{\CLoopL[#1]{90}{#2}{#3}}
\newcommand{\CLoopS}[3][{\CLoopLblPos}]{\CLoopR[#1]{-90}{#2}{#3}}
\newcommand{\CLoopNW}[3][{\CLoopLblPos}]{\CLoopR[#1]{135}{#2}{#3}}
\newcommand{\CLoopNE}[3][{\CLoopLblPos}]{\CLoopL[#1]{45}{#2}{#3}}
\newcommand{\CLoopSW}[3][{\CLoopLblPos}]{\CLoopL[#1]{-135}{#2}{#3}}
\newcommand{\CLoopSE}[3][{\CLoopLblPos}]{\CLoopR[#1]{-45}{#2}{#3}}
\newcommand{\LoopVarN}[3][{\CLoopLblPos}]{\LoopVarL[#1]{90}{#2}{#3}}
\newcommand{\LoopVarS}[3][{\CLoopLblPos}]{\LoopVarR[#1]{-90}{#2}{#3}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%\section{backward compatibility}%%%%%%
%%%%%  Obsolete commands from version 0.3, 0.4 and 1.0
%%%%%  kept for backward compatibility
%%%%%  cf users manual for description of compatibilty problems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ReverseArrow}{\ReverseTransitions}%
\newcommand{\StraightArrow}{\DirectTransitions}%
\newcommand{\FixDimEdge}[4]{\SetDimEdgePmts{#1}{#2}{#3}{#4}}%
\newcommand{\EdgeBorder}{\EdgeLineBorderOn}%
\newcommand{\EdgeBorderOff}{\EdgeLineBorderOff}%
\newcommand{\FixEdgeBorder}[2]{\FixEdgeLineBorder{#1}{#2}}%
\newcommand{\ForthBackOffset}{\ForthBackOffsetOn}%
%
\newcommand{\SetEdgeArrowWidth}[1]{\SetEdgeArrowWidthBase{#1}}			%width of the edge arrow
\newlength{\EdgeDblArrowWidth}		%width : 
\setlength{\EdgeDblArrowWidth}{1.3mm}		%width : 
\newcommand{\EdgeDblArrowLengthCoef}{}	% 
%
\newcommand{\EdgeLabelPosit}{}\newcommand{\EdgeLabelRevPosit}{}
\newcommand{\ArcLabelPosit}{}\newcommand{\ArcLabelRevPosit}{}
\newcommand{\LArcLabelPosit}{}\newcommand{\LArcLabelRevPosit}{}
\newcommand{\LoopLabelPosit}{}\newcommand{\LoopLabelRevPosit}{}
\newcommand{\CLoopLabelPosit}{}\newcommand{\CLoopLabelRevPosit}{}
%
\newcommand{\LoopVarAngle}{}\newcommand{\LoopVarAng}{}
\newcommand{\LoopVarSize}{}\newcommand{\LoopVarSi}{}
\newlength{\LoopVarOffset}\newlength{\LoopVarOff}
\newcommand{\LoopOnVariableState}{} 
\newcommand{\CLoopOnVariableState}{}
\newcommand{\LoopOnVerySmallState}{} 
%
\newcommand{\ChgLoopVarSize}[1]{\renewcommand{\LoopVarSi}{#1}}
\newcommand{\RstLoopVarSize}{\ChgLoopVarSize{\LoopVarSize}}
\newcommand{\SetLoopVarSize}[1]%
   {\renewcommand{\LoopVarSize}{#1}\RstLoopVarSize}
% label position on initial-final arrow
\newcommand{\InitStateLabelPosit}{}\newcommand{\InitStateLabelRevPosit}{}
\newcommand{\FinalStateLabelPosit}{}\newcommand{\FinalStateLabelRevPosit}{}
%
\newcommand{\ArrowOnVerySmallState}{5} 
%
\newcommand{\VArcL}[5][{\ArcLblPos}]%
   {\EdgeStyle \ArcLStyle%\psset{style=VaucLArcL} 
    \ncarc[#2]{#3}{#4} \WRLLbl{#1}{#5}}%\naput[npos=#1]{\VaucEdgeLabel{#5}}
\newcommand{\VArcR}[5][{\ArcLblPos}]%
   {\EdgeStyle \ArcRStyle%\psset{style=VaucLArcR} 
    \ncarc[#2]{#3}{#4} \WRRLbl{#1}{#5}}%\nbput[npos=#1]{\VaucEdgeLabel{#5}}
%
\newcommand{\VCurveL}[5][{\ArcLblPos}]%
   {\EdgeStyle \psset{angleA=0,angleB=180,ncurv=1}% 
    \nccurve[#2]{#3}{#4} \WRLLbl{#1}{#5}}%\naput[npos=#1]{\VaucEdgeLabel{#5}}
\newcommand{\VCurveR}[5][{\ArcLblPos}]%
   {\EdgeStyle \psset{angleA=0,angleB=0,ncurv=1}% 
    \nccurve[#2]{#3}{#4} \WRRLbl{#1}{#5}}%\nbput[npos=#1]{\VaucEdgeLabel{#5}}
%
\newcommand{\LabelL}[2][{\EdgLblPos}]{\WRLLbl{#1}{#2}}%\naput[npos=#1]{\VaucEdgeLabel{#2}}
\newcommand{\LabelR}[2][{\EdgLblPos}]{\WRRLbl{#1}{#2}}%\nbput[npos=#1]{\VaucEdgeLabel{#2}}
%%%  Initial-final quality: obsolete as the phantom positions are not 
%%%  generated anymore
\newcommand{\VCIFflag}{2}\newcommand{\VCIFflagtemp}{2}
\newcommand{\PlainState}{}%
\newcommand{\FullState}{}%
\newcommand{\IFState}{}
\newcommand{\IFXState}{}
\newcommand{\RstVCIF}{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
arrows=\EdgeArrowSty,%
arrowsize=\EdgArrowWidthDim,%
arrowlength=\EdgArrowLengthCoef,%
arrowinset=\EdgArrowInsetCoef,%
\newcommand{\SetEdgArrowWD}% internal function
   {\setlength{\EdgArrowWidthDim}{\EdgArrowWDBase}%
    \addtolength{\EdgArrowWidthDim}{\EdgArrowWidthCoef\EdgeLineWid}}
\newcommand{\SetDblEdgArrowWD}% internal function
   {\setlength{\DblEdgArrowWidthDim}{\DblEdgArrowWDBase}%
    \addtolength{\DblEdgArrowWidthDim}%
                {\DblEdgArrowWidthCoef\DblEdgLineWD}}


==> VCSG-environment.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:    VCSG-environment
%%
%% DESCRIPTION:  Definition of the picture environment
%%
%% DATE:    2008/12/28
%%
%% Copyright (C) 2009 Sylvain Lombardy and Jacques Sakarovitch
%    2.1 - 050219
%    2.2 - 050727
%    2.3 - 060628     Modif. induced by VCSG-edgess
%          091016     \VCInputFig added
%          091028     Calls for version compatibility and 
%                     initialisation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Scaling matters}%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% "Sizes" (eg for states) and "widths" (of lines) are given 
%%% as "lengthes" in a fixed unit (cm or pt), 
%%% whereas the positions are normally given in "psunits".
%%% 
%%% This allows to use different scaling parameters 
%%% for the whole figure and for the "drawing grid".
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scaling parameters
\newcommand{\VCScale}{}%      Global scale parameter
\newcommand{\VCGridScale}{}%  Grid scale parameter
\newcommand{\LargeScale}{}%   Preset value
\newcommand{\MediumScale}{}%  Preset value
\newcommand{\SmallScale}{}%   Preset value
\newcommand{\TinyScale}{}%    Preset value
\newcommand{\LargeScaleI}{}%   Preset value
\newcommand{\MediumScaleI}{}%  Preset value
\newcommand{\SmallScaleI}{}%   Preset value
\newcommand{\TinyScaleI}{}%    Preset value
%%% Scaling commands
% general
\newcommand{\FixVCScale}[1]{\renewcommand{\VCScale}{#1}}% 
\newcommand{\FixVCGridScale}[1]{\renewcommand{\VCGridScale}{#1}}%
\newcommand{\FixPctScale}[2]%
   {\renewcommand{\VCScale}{#1}%
    \SetStateLabelScale{#2}%
    \SetEdgeLabelScale{#2}%
    \FixVCGridScale{1}%
   }% 
% with preset parameters
\newcommand{\LargePictures}{\FixPctScale{\LargeScale}{\LargeScaleI}}
\newcommand{\MediumPictures}{\FixPctScale{\MediumScale}{\MediumScaleI}}
\newcommand{\SmallPictures}{\FixPctScale{\SmallScale}{\SmallScaleI}}
\newcommand{\TinyPictures}{\FixPctScale{\TinyScale}{\TinyScaleI}}
% for compatibility
\newcommand{\LargePicture}{\FixVCScale{\LargeScale}\FixVCGridScale{1}}
\newcommand{\MediumPicture}{\FixVCScale{\MediumScale}\FixVCGridScale{1}}
\newcommand{\SmallPicture}{\FixVCScale{\SmallScale}\FixVCGridScale{1}}
\newcommand{\TinyPicture}{\FixVCScale{\TinyScale}\FixVCGridScale{1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Picture directory}%%%%%
\newcommand{\VCDirectory}{}% the definition is an initialisation
\newcommand{\SetVCDirectory}[1]{\renewcommand{\VCDirectory}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Picture framing}%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% flags 
\newif\ifVCFrame% showing/hiding the frame "around" the picture
\newcommand{\HideFrame}{\VCFramefalse}
\newcommand{\ShowFrame}{\VCFrametrue}
\newif\ifVCGrid% showing/hiding the grid in the frame
\newcommand{\HideGrid}{\VCGridfalse}
\newcommand{\ShowGrid}%
   {\VCGridtrue%
    \renewcommand{\VCGridLabelColor}{\VCGridLineColor}}
\newcommand{\ShowGridNL}%
   {\VCGridtrue%
    \renewcommand{\VCGridLabelColor}{white}}
\newif\ifVCName% printing/or not the name of the figure file
\newcommand{\HideName}{\VCNamefalse}
\newcommand{\ShowName}{\VCNametrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  inner parameters (no doubling)
\newcommand{\VCBkgdStyle}{}
\newcommand{\VCBkgdColor}{}
\newcommand{\SetVCBkgdStyle}[1]%% ATTN Reset Bkgd for states
    {\renewcommand{\VCBkgdStyle}{#1}%
     \SetStateBkgdStyle{#1}}
\newcommand{\SetVCBkgdColor}[1]%% ATTN Reset Bkgd for states
    {\renewcommand{\VCBkgdColor}{#1}%
     \SetStateBkgdColor{#1}%
     \renewcommand{\SttBorderColor}{#1}% Border -- see VCSG-states
     \SetEdgeLineBorderColor{#1}% Border -- see VCSG-edges
     \SetDblEdgeLineColor{#1}% double lines -- see VCSG-edges
    }%
% (to be changed with a \renewcommand)
\newlength{\VCFrameLineWidth}{}
\newcommand{\VCFrameLineColor}{}
\newlength{\VCGridLineWidth}{}
\newcommand{\VCGridLineColor}{}
\newcommand{\VCGridLabelColor}{}% in view of \ShowGridNL
\newcommand{\VCSubGridLineColor}{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   styles for the background, frame and grid 
\newpsstyle{VCBkgdStyle}%
           {framesep=0pt,
            arrows=-,%                   
            linestyle=none,%
            linewidth=0.1pt,
            linecolor=black,%
            doubleline=false,%
            dimen=inner,% the frame has exactly the given size
            fillcolor=\VCBkgdColor,%
            fillstyle=\VCBkgdStyle,%
            griddots=0,% no grid a priori
            cornersize=relative,%
            framearc=0}
\newpsstyle{VCFrameStyle}% to be used just after VCBkgdStyle
           {linestyle=solid,%
            linewidth=\VCFrameLineWidth,%
	    linecolor=\VCFrameLineColor,%
            doubleline=false}%,
\newpsstyle{VCGridStyle}% to be used just after VCFrameStyle
           {gridwidth=\VCGridLineWidth,%
            griddots=10,%
	    gridcolor=\VCGridLineColor,%
            gridlabels=7pt,%
            gridlabelcolor=\VCGridLabelColor,%
            subgridwidth=0.2pt,%
            subgriddiv=5,%
            subgridcolor=\VCSubGridLineColor}
\newcommand{\BkgdStyle}{\psset{style=VCBkgdStyle}}
\newcommand{\FrameStyle}{\psset{style=VCFrameStyle}}
\newcommand{\GridStyle}%
   {\ifthenelse{\equal{\VCGridLineColor}{black}}% 
       {\renewcommand{\VCSubGridLineColor}{black}}%
       {\renewcommand{\VCSubGridLineColor}{\VCGridLineColor}}%
    \psset{style=VCGridStyle}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Picture drawing call}%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In order to make the parameter VCScale part of the environment and 
% dealt with by VauCanSon-G commands, the call look like:
%
%  \VCDraw{%
%     \begin{VCPicture}{(x0,y0)(x1,y1)}
%     %  figure description ...
%     \end{VCPicture}%
%    }
%
% or like
%
% \VCCall{figure-file-name}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  parameters
\newlength{\VCSGMinHeight}%
\newlength{\VCSGMaxHeight}%
\newcommand{\VCVertPlac}{}%
\newcommand{\FixVerticalPlacement}[1]{\renewcommand{\VCVertPlac}{#1}}
%%%  picture environment
\newenvironment{VCPicture}[2][\VCVertPlac]%
  {%
   \pssetlength{\VCSGMinHeight}{\VCSGProjectionOnSecondComponent#2}%
   \pssetlength{\VCSGMaxHeight}{\VCSGProjectionOnFourthComponent#2}%
   \addtolength{\VCSGMinHeight}{-\VCSGMaxHeight}%
   \begin{pspicture}[shift=#1\VCSGMinHeight]#2%
       \BkgdStyle \psframe#2%
       \ifVCFrame \FrameStyle \psframe#2\fi%
       \ifVCGrid  \FrameStyle \GridStyle \psgrid#2\fi}%
  {\RstState
% %     \RstVertex%
% %     \RstEdge%
   \end{pspicture}}%
%%%  calls to the picture environment
\newcommand{\VCDraw}[2][\VCGridScale]%
   {\psset{unit=#1cm}%
    \scalebox{\VCScale}{#2}%
    \psset{unit=\VCGridScale cm}}
%
\newcommand{\VCCall}[2][\VCGridScale]%
   {\psset{unit=#1cm}%
    \ifVCName\makebox[0pt][r]{\fbox{{\scriptsize #2}}}\fi%
    \scalebox{\VCScale}{\input{\VCDirectory #2}}%
    \psset{unit=\VCGridScale cm}}
%%%  call to part of a picture
% Allows to put parts of figures in the \VCDirectory 
% and to call them inside a \VCDraw
\newcommand{\VCInputFig}[1]{\input{\VCDirectory #1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{VauCanSon-G modes}%%%%%
\newcommand{\VCMode}{}  
\newcommand{\Automata}%
   {\renewcommand{\VCMode}{automata}\SizedNodes}
\newcommand{\Graphs}%
   {\renewcommand{\VCMode}{graphs}\SizelessNodes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Version compatibility}%%%%%
\newcommand{\VCSGZeroFour}{\input VCPref-version04.tex }
\newcommand{\VCSGOne}{\input VCPref-version1.tex }
\newcommand{\VCSGInit}{\input VCSG-Preferences.tex }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> VCSG-functions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:    VCSG-functions.tex
%%
%% DESCRIPTION:
%%
%%   Auxiliary functions and variables called inside VauCanSon-G 
%%   PSTricks commands to be used inside pictures with VauCanSon-G's 
%%   syntax 
%%  
%% DATE:    2008/12/28
%%
%% Copyright (C) 2009 Sylvain Lombardy and Jacques Sakarovitch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{constants}%%%%%%%%
\newcommand{\VCSG}
     {\textsc{V$\overline{\text{au}}$%
              C\raisebox{.3ex}{$\underline{\text{an}}$}%
              S$\overline{\text{on}}$-G}\xspace}
\newcommand{\vcsg}
     {\textsc{V$\overline{\text{cs}}$G}\xspace}
\newcommand{\Vaucanson}{\VCSG}% compatibility (with what??)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Constants for geometric constructions
\newcommand{\HSQRTwo}{0.717}
\newcommand{\SQRThree}{1.732}
\newcommand{\GoldMean}{0.618}
\newcommand{\GoldMeanI}{1.618}
\newcommand{\SQRGoldMeanI}{1.272}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% If it has to be somewhere before the preferences, here is the best
\psset{unit=1cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{constants}%%%%%%%%
\newlength{\VCSGTmpLength}
\newlength{\VCSGTmpLengthbis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{functions}%%%%%%%%
\def\VCSGProjectionOnSecondComponent(#1,#2)(#3,#4){#2}%
\def\VCSGProjectionOnFourthComponent(#1,#2)(#3,#4){#4}%
%%% Functions for dealing with numbers
\newcommand{\VCSGCmdPosTst}[1]{\lengthtest{#1pt > 0pt}}
\newcommand{\VCSGGreaterLgt}[3]%
    {\ifthenelse{\lengthtest{#1 > #2}\or\lengthtest{#1 = #2}}%
        {\setlength{#3}{#1}}%
        {\setlength{#3}{#2}}%
     }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Functions for geometric constructions
\newcommand{\VCSGCompassDecode}[2]%
% Translate the eight compass directions into degrees
% If #1 is not a compass direction, simply copy it into #2
   {\ifthenelse{\equal{#1}{n}}%#2
       {\renewcommand{#2}{90}}%
       {\ifthenelse{\equal{#1}{ne}}%
           {\renewcommand{#2}{45}}%
           {\ifthenelse{\equal{#1}{e}}%
               {\renewcommand{#2}{0}}%
               {\ifthenelse{\equal{#1}{se}}%
                   {\renewcommand{#2}{315}}%
                   {\ifthenelse{\equal{#1}{s}}%
                       {\renewcommand{#2}{270}}%
                       {\ifthenelse{\equal{#1}{sw}}%
                           {\renewcommand{#2}{225}}%
                           {\ifthenelse{\equal{#1}{w}}%
                               {\renewcommand{#2}{180}}%
                               {\ifthenelse{\equal{#1}{nw}}%
                                   {\renewcommand{#2}{135}}%
                                   {\renewcommand{#2}{#1}}}}}}}}}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{PSTricks commands}
\newcommand{\Point}[2]{\pnode#1{#2}}
\newcommand{\VCPut}[3][0]{\rput{#1}#2{#3}}% 
\newcommand{\Translate}[2]{\rput#1{#2}}% 
\newcommand{\Rotate}[2]{\rput{#1}(0,0){#2}}% 
\newcommand{\TransRotate}[3]{\rput{#2}#1{#3}}% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%\section{backward compatibility}%%%%%%
\newcommand{\SQRTwo}{0.717}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> VCSG-states.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:    VCSG-states.tex
%%
%% DESCRIPTION:   Commands for drawing states
%%
%% DATE:    2009/01/06
%%
%% Copyright (C) 2009 Sylvain Lombardy and Jacques Sakarovitch
%    2.1 - 05/02/19
%    2.2 - 05/03/02    VCS-states
%    2.3 - 05/07/29    include VCS-state-labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Node mode}%%%%%%
%%% A flag to distinguish between "sized" and "sizeless" nodes
\newif\ifVCSizedNode   
\newcommand{\SizedNodes}{\VCSizedNodetrue}
\newcommand{\SizelessNodes}{\VCSizedNodefalse}
%%% synonymous
\newcommand{\SizedStates}{\SizedNodes}
\newcommand{\SizelessStates}{\SizelessNodes}
\newcommand{\SizedVertices}{\SizedNodes}
\newcommand{\SizelessVertices}{\SizelessNodes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state size}%%%%%%
%%%  A variable to remember the current size of states
\newcommand{\VCSttSize}{}
% VSState (very small state) does not change the value:
%                                 it is not a mode that is remembered
%  That variable allows to fix (via preset values) such parameters as
%  the lenght of initial or final arrows and 
%  the curvature and offset of loops 
%  No effect on Vertex
% %%% Size = StateSize
%%% mod. 2.3  change to a more logical terminology
%%% The `size' of a state is `small', `medium' or `large'
%%% The `diameter' of a state is a length.
\newlength{\StateDiameter}\newlength{\StateDia}
%%%   Preset size parameters
%%% The preset sizes are given in cm, and not in "psunits".
%%% This allows to use different scales for the whole figure 
%%% and for the "drawing grid".
\newlength{\MediumStateDiameter}
\newlength{\SmallStateDiameter}
\newlength{\LargeStateDiameter}
\newlength{\VerySmallStateDiameter}% may be to be moved
%%%
\newcommand{\FixStateSizes}[4]% 
   {\setlength{\SmallStateDiameter}{#1}%
    \setlength{\MediumStateDiameter}{#2}%
    \setlength{\LargeStateDiameter}{#3}%
    \setlength{\VerySmallStateDiameter}{#4}}
%%% Changes of the state diameter as it is commonly provided for other 
%%% parameters 
%%% is not recommanded for it should be accompanied by a modification
%%% of many other parameters (for the drawing of arcs and loops).
%%% and this is what the above commands are made for. ?????
%%% However it may be useful in some cases to be able to modify 
%%% the state diameter and we thus have the same set of commands as 
%%% for other parameters (the use of `Stt' instead of `State' is 
%%% supposed to be a reminder that they are almost
%%% internal commands.
\newcommand{\ChgSttDiameter}[1]{\setlength{\StateDia}{#1\StateDiameter}}  
\newcommand{\RstSttDiameter}{\ChgSttDiameter{1}}
\newcommand{\SetSttDiameter}[1]% 
   {\setlength{\StateDiameter}{#1}\RstSttDiameter}
\newcommand{\IncChgSttDiameter}[1]{\setlength{\StateDia}{#1\StateDia}}  
% 
\newcommand{\FixStateDiameter}[1]{\SetSttDiameter{#1}}  
%%% setting state size, and the other parameters that come along
\newcommand{\EstabSttSize}[5]%
   {%
    \renewcommand{\VCSttSize}{#1}%
    \SetSttDiameter{#2}%
    \renewcommand{\ArrowOnStateCoef}{#3}% en attendant la partie 
                                        % inital-final
    \SetLoopSize{#4}%         en attendant la partie edges
%     \SetLoopVarSize{#4}%
    \SetCLoopSize{#5}%
   }
%%%
\newcommand{\MediumStates}%
   {\EstabSttSize{medium}{\MediumStateDiameter}{\ArrowOnMediumState}%
	       {\LoopOnMediumState}{\CLoopOnMediumState}}
\newcommand{\SmallStates}%
   {\EstabSttSize{small}{\SmallStateDiameter}{\ArrowOnSmallState}%
               {\LoopOnSmallState}{\CLoopOnSmallState}}
\newcommand{\LargeStates}%
   {\EstabSttSize{large}{\LargeStateDiameter}{\ArrowOnLargeState}%
               {\LoopOnLargeState}{\CLoopOnLargeState}}
%%% recovering the current preset value for size
\newcommand{\RstStateSize}%
  {\ifthenelse{\equal{\VCSttSize}{medium}}%
              {\MediumStates}%
              {\ifthenelse{\equal{\VCSttSize}{small}}%
                          {\SmallStates}%
			  {\ifthenelse{\equal{\VCSttSize}{large}}%
			              {\LargeStates}{ErrStateSize}}}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state shape}%%%%%
%%%  A variable to remember the current shape of states
\newcommand{\VCSttShape}{}% remember the current shape of states
\newcommand{\VCSttShp}{}%   int. var. used when state is processed
% 
\newcommand{\CircleStates}{\renewcommand{\VCSttShape}{circle}}
\newcommand{\OvalStates}{\renewcommand{\VCSttShape}{oval}}
\newcommand{\SquareStates}{\renewcommand{\VCSttShape}{square}}
\newcommand{\RectangleStates}{\renewcommand{\VCSttShape}{rectangle}}
%%% shape of oval states
\newcommand{\OvalStateRatio}{}\newcommand{\OvalStateRat}{}
% changing/setting the shape of rectangular states
\newcommand{\ChgOvalStateRatio}[1]{\renewcommand{\OvalStateRat}{#1}}
\newcommand{\RstOvalStateRatio}%
   {\ChgOvalStateRatio{\OvalStateRatio}}
\newcommand{\SetOvalStateRatio}[1]%
   {\renewcommand{\OvalStateRatio}{#1}\RstOvalStateRatio}
%%% shape of rectangular states
\newcommand{\RectangleStateRatio}{}\newcommand{\RectangleStateRat}{}
% changing/setting the shape of rectangular states
\newcommand{\ChgRectangleStateRatio}[1]{\renewcommand{\RectangleStateRat}{#1}}
\newcommand{\RstRectangleStateRatio}%
   {\ChgRectangleStateRatio{\RectangleStateRatio}}
\newcommand{\SetRectangleStateRatio}[1]%
   {\renewcommand{\RectangleStateRatio}{#1}\RstRectangleStateRatio}
%%%  Rounding the corners of square/rectangular states
%  A flag to remember the rounding of square/rectangular states
\newif\ifRoundedState%
%%%  The rounding may be `relative' or `absolute'
%%%  Variables that follow record the mode of rounding and the 
%%%  corresponding parameters
\newcommand{\StateCornerRounding}{}% record the mode of rounding
% Setting the mode of rounding
\newcommand{\StateCornerRoundingAbsolute}%
   {\renewcommand{\StateCornerRounding}{absolute}}
\newcommand{\StateCornerRoundingRelative}%
   {\renewcommand{\StateCornerRounding}{relative}}
%  Relative rounding. Radius for rounded corners is a float
%                     Will be given in the psstyle as "framearc"
\newcommand{\StateCornerRelRadius}{}\newcommand{\StateCornerRelRad}{}
%   ATTN   Relative radius is "changed" "absolutely"
\newcommand{\ChgStateCornerRelRadius}[1]%
   {\renewcommand{\StateCornerRelRad}{#1}}
\newcommand{\RstStateCornerRelRadius}%
   {\ChgStateCornerRelRadius{\StateCornerRelRadius}}
\newcommand{\SetStateCornerRelRadius}[1]%
   {\renewcommand{\StateCornerRelRadius}{#1}\RstStateCornerRelRadius}
%  Absolute rounding. Radius for rounded corners is a length
%                     Will be given in the psstyle as "linearc"
%     Together with the usual 2 variables, xxxRadius and xxxRad, a 
%     third one, xxxRadEff, is the one that is given to the psstyle 
%     and allows to switch between sharp and rounded states without 
%     interfering wwith the normal process of rounded states
\newlength{\StateCornerRadius}\newlength{\StateCornerRad}
\newlength{\StateCornerRadEff}
%
\newcommand{\ChgStateCornerRadius}[1]%
   {\setlength{\StateCornerRad}{#1\StateCornerRadius}%
    \ifRoundedState\setlength{\StateCornerRadEff}{\StateCornerRad}\fi}
\newcommand{\RstStateCornerRadius}{\ChgStateCornerRadius{1}}
\newcommand{\SetStateCornerRadius}[1]%
   {\setlength{\StateCornerRadius}{#1}\RstStateCornerRadius}
% Switching between sharp and rounded corners
\newcommand{\SharpStateCorners}%
   {\RoundedStatefalse\setlength{\StateCornerRadEff}{0pt}}
\newcommand{\RoundedStateCorners}%
   {\RoundedStatetrue\setlength{\StateCornerRadEff}{\StateCornerRad}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Hiding -- showing}%%%%%
%%% Hiding -- showing states (used for overlays in slides)
% (used internally for the hidden states in adjusted states) 
% the trick is to have two different styles instead of 
% saving\restoring parameters
\newif\ifVCShowStt
\newcommand{\HideStates}{\VCShowSttfalse}
\newcommand{\ShowStates}{\VCShowStttrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state background parameters}%%%%%
\newcommand{\StateBkgdStyle}{}\newcommand{\StateBkgdSty}{} 
\newcommand{\StateBkgdColor}{}\newcommand{\StateBkgdCol}{}
   % As they have usually no labels it useful
   % to have a special coloring facility for the "SmallState"
   % especially for slide style
\newcommand{\SmallStateBkgdStyle}{}
\newcommand{\SmallStateBkgdColor}{} 
%%%  changing/setting macros
% changing/setting the background style 
\newcommand{\ChgStateBkgdStyle}[1]{\renewcommand{\StateBkgdSty}{#1}}
\newcommand{\RstStateBkgdStyle}{\ChgStateBkgdStyle{\StateBkgdStyle}}
\newcommand{\SetStateBkgdStyle}[1]% 
    {\renewcommand{\StateBkgdStyle}{#1}\RstStateBkgdStyle%
     \renewcommand{\SmallStateBkgdStyle}{#1}% ATTN reset Bkgd for 
                                            % Small States
    }
% changing/setting the background color 
\newcommand{\ChgStateBkgdColor}[1]{\renewcommand{\StateBkgdCol}{#1}}
\newcommand{\RstStateBkgdColor}{\ChgStateBkgdColor{\StateBkgdColor}}
\newcommand{\SetStateBkgdColor}[1]% 
    {\renewcommand{\StateBkgdColor}{#1}\RstStateBkgdColor%
     \renewcommand{\SmallStateBkgdColor}{#1}% ATTN reset Bkgd for 
                                            % Small States
    }
% setting SmallState background style and color 
\newcommand{\SetSmallStateBkgdStyle}[1]%
    {\renewcommand{\SmallStateBkgdStyle}{#1}}
\newcommand{\SetSmallStateBkgdColor}[1]%
    {\renewcommand{\SmallStateBkgdColor}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state line parameters}%%%%%%
\newlength{\StateLineWidth}\newlength{\StateLineWid}
% \newcommand{\VSStateLineCoef}{} % coef. for very small state
\newcommand{\StateLineStyle}{}\newcommand{\StateLineSty}{} 
\newcommand{\StateLineColor}{}\newcommand{\StateLineCol}{}
% parameters for double line
\newif\ifStateLineDbl 
\newcommand{\StateLineDbl}{} 
\newcommand{\SttLineDblCoef}{} 
\newcommand{\StateLineDblColor}{} 
\newcommand{\SttLineDblSep}{}\newcommand{\StateLineDblSp}{} 
% internal parameters
\newcommand{\SttDimen}{} 
\newcommand{\SttDblLineDimen}{}
% Border (of prescribed width and color) on both side of the line for 
% giving  the impression that one line passes above another. 
% May be useful when transitions cross over (under) states, but this 
% is not likely to happen so often.
\newlength{\SttBorderWidth}
\newcommand{\SttBorderColor}{}% normally same as state Bkgd
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  changing/setting macros 
% changing/setting the width of state line 
\newcommand{\ChgStateLineWidth}[1]%
   {\setlength{\StateLineWid}{#1\StateLineWidth}}  
\newcommand{\RstStateLineWidth}{\ChgStateLineWidth{1}}
\newcommand{\SetStateLineWidth}[1]% ATTN the parameter is a length
   {\setlength{\StateLineWidth}{#1}\RstStateLineWidth}
% changing/setting the style of state line 
\newcommand{\ChgStateLineStyle}[1]{\renewcommand{\StateLineSty}{#1}}
\newcommand{\RstStateLineStyle}{\ChgStateLineStyle{\StateLineStyle}}
\newcommand{\SetStateLineStyle}[1]%
   {\renewcommand{\StateLineStyle}{#1}\RstStateLineStyle}
% changing/setting the color of state line
\newcommand{\ChgStateLineColor}[1]{\renewcommand{\StateLineCol}{#1}}
\newcommand{\RstStateLineColor}{\ChgStateLineColor{\StateLineColor}}
\newcommand{\SetStateLineColor}[1]%
   {\renewcommand{\StateLineColor}{#1}\RstStateLineColor}
% changing/setting the doubleline status
\newcommand{\StateLineDouble}%
    {\StateLineDbltrue\renewcommand{\StateLineDbl}{true}}
\newcommand{\StateLineSimple}%
    {\StateLineDblfalse\renewcommand{\StateLineDbl}{false}}
%%%
\newcommand{\FixStateLineDouble}[2]%
   {\renewcommand{\SttLineDblCoef}{#1}%
    \renewcommand{\SttLineDblSep}{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{State drawing style}%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Switching between simple and double line is made by adding style,
% not by setting parameters
\newpsstyle{VCStateStyle}%
        {framesep=0pt,%
         fillstyle=\StateBkgdSty,%
	 fillcolor=\StateBkgdCol,% 
         linewidth=\StateLineWid,%
	 linestyle=\StateLineSty,%
	 linecolor=\StateLineCol,%
         border=\SttBorderWidth,%
         bordercolor=\SttBorderColor,%
	 dimen=\SttDimen,%
         doubleline=false,%\StateLineDbl
         cornersize=\StateCornerRounding,%
	 linearc=\StateCornerRadEff,%
	 framearc=\StateCornerRelRad}
\newpsstyle{VCStateDblStyle}% ATTN New version: incremental style
        {%                   
	 doubleline=true,%\StateLineDbl
         linewidth=\SttLineDblCoef\StateLineWid,%
	 doublesep=\SttLineDblSep\StateLineWid,%
	 doublecolor=\StateBkgdCol,%
	 dimen=\SttDblLineDimen}
\newpsstyle{VCHiddenStateStyle}% ATTN New version: incremental style
        {%                   
         linestyle=none,%
         fillstyle=none}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% new version
\newcommand{\SttStyle}%
   {%
    \ifthenelse{\equal{\VCSttSize}{small}}% 
       {\renewcommand{\StateBkgdSty}{\SmallStateBkgdStyle}%
        \renewcommand{\StateBkgdCol}{\SmallStateBkgdColor}}%
       {}%  
    \psset{style=VCStateStyle}%
    \ifStateLineDbl\psset{style=VCStateDblStyle}\fi%
    \ifVCShowStt\else\psset{style=VCHiddenStateStyle}\fi%
   }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% TO BE FIXED
%%%   Variable state with double line
%%%   may change the policy of drawing states with double line
%%%   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% VCSG-state-labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state label parameters}%%%%%
% flags
\newif\ifVCRigidStateLabel
\newcommand{\RigidStateLabel}{\VCRigidStateLabeltrue}
\newcommand{\SwivelStateLabel}{\VCRigidStateLabelfalse}
\newif\ifVCStateLabelOnBaseLine
\newcommand{\AlignedStateLabel}{\VCStateLabelOnBaseLinetrue}
\newcommand{\FloatingStateLabel}{\VCStateLabelOnBaseLinefalse}
\newif\ifVCStateLabelInside
\newcommand{\StateLabelInside}{\VCStateLabelInsidetrue}
\newcommand{\StateLabelAside}{\VCStateLabelInsidefalse}
% parameters
\newcommand{\StateLabelColor}{}\newcommand{\StateLabelCol}{}
\newcommand{\StateLabelScale}{}\newcommand{\StateLabelSca}{}
\newcommand{\StateLabelSize}{}\newcommand{\StateLabelSz}{}
\newcommand{\StateLabelStyle}{}\newcommand{\StateLabelSty}{}
% 050302 text mode
\newcommand{\SttLblMode}{} % Internal variable
% parameters for aside labels
\newcommand{\AsideLabelDirct}{}\newcommand{\AsideLabelDir}{}
\newlength{\AsideLabelDistn}{}\newlength{\AsideLabelDst}{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state label changing/setting macros}%%%%%
% changing/setting the label color
\newcommand{\ChgStateLabelColor}[1]{\renewcommand{\StateLabelCol}{#1}}
\newcommand{\RstStateLabelColor}{\ChgStateLabelColor{\StateLabelColor}}
\newcommand{\SetStateLabelColor}[1]%
    {\renewcommand{\StateLabelColor}{#1}\RstStateLabelColor}
% changing/setting the label scale
\newcommand{\ChgStateLabelScale}[1]{\renewcommand{\StateLabelSca}{#1}}
\newcommand{\RstStateLabelScale}{\ChgStateLabelScale{1}}
\newcommand{\SetStateLabelScale}[1]%
   {\renewcommand{\StateLabelScale}{#1}\RstStateLabelScale}
% changing/setting the label size
\newcommand{\ChgStateLabelSize}[1]{\renewcommand{\StateLabelSz}{#1}}
\newcommand{\RstStateLabelSize}{\ChgStateLabelSize{\StateLabelSize}}
\newcommand{\SetStateLabelSize}[1]%
    {\renewcommand{\StateLabelSize}{#1}\RstStateLabelSize}
% changing/setting the label style
\newcommand{\ChgStateLabelStyle}[1]{\renewcommand{\StateLabelSty}{#1}}
\newcommand{\RstStateLabelStyle}{\ChgStateLabelStyle{\StateLabelStyle}}
\newcommand{\SetStateLabelStyle}[1]%
    {\renewcommand{\StateLabelStyle}{#1}\RstStateLabelStyle}
% setting the label text mode %%% processed differently
\newcommand{\StateLabelModeMath}{\renewcommand{\SttLblMode}{$}}%
\newcommand{\StateLabelModeText}{\renewcommand{\SttLblMode}{}}%
% changing/setting the direction of the label aside
\newcommand{\ChgAsideLabelDirct}[1]{\renewcommand{\AsideLabelDir}{#1}}
\newcommand{\RstAsideLabelDirct}{\ChgAsideLabelDirct{\AsideLabelDirct}}
\newcommand{\SetAsideLabelDirct}[1]%
   {\renewcommand{\AsideLabelDirct}{#1}\RstAsideLabelDirct}
% changing/setting the distance of the label aside 
\newcommand{\ChgAsideLabelDistn}[1]%
   {\setlength{\AsideLabelDst}{#1\AsideLabelDistn}}  
\newcommand{\RstAsideLabelDistn}{\ChgAsideLabelDistn{1}}
\newcommand{\SetAsideLabelDistn}[1]% ATTN the parameter is a length
   {\setlength{\AsideLabelDistn}{#1}\RstAsideLabelDistn}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{dimmed states}%%%%
%%%  Dimmed states (e.g. for non accessible states)
\newcommand{\DimStateLineStyle}{} 
\newcommand{\DimStateLineCoef}{} 
\newcommand{\DimStateLineColor}{}
\newcommand{\DimStateBkgdColor}{}
\newcommand{\DimStateLabelColor}{}
%%% establishing the dimmed style
\newcommand{\DimState}%
   {\ChgStateLineStyle{\DimStateLineStyle}%
    \ChgStateLineWidth{\DimStateLineCoef}%
    \ChgStateLineColor{\DimStateLineColor}%
    \ChgStateBkgdColor{\DimStateBkgdColor}%
    \ChgStateLabelColor{\DimStateLabelColor}}
%
\newcommand{\SetDimStatePmts}[5]%
   {\renewcommand{\DimStateLineStyle}{#1}%
    \renewcommand{\DimStateLineCoef}{#2}%
    \renewcommand{\DimStateLineColor}{#3}%
    \renewcommand{\DimStateLabelColor}{#4}%
    \renewcommand{\DimStateBkgdColor}{#5}%
    \renewcommand{\DimState}%
       {\ChgStateLineStyle{\DimStateLineStyle}%
        \ChgStateLineWidth{\DimStateLineCoef}%
        \ChgStateLineColor{\DimStateLineColor}%
        \ChgStateBkgdColor{\DimStateBkgdColor}%
        \ChgStateLabelColor{\DimStateLabelColor}}%
    }
%
\newcommand{\UnDimState}%
   {\RstStateLineStyle%
    \RstStateLineWidth%
    \RstStateLineColor%
    \RstStateBkgdColor%
    \RstStateLabelColor}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% restoring state parameters and thus 
%%% initializing the internal parameters to the default values
%%% TO BE FIXED  The initial values of the flags are not stored
%%%              and thus not restored
\newcommand{\RstState}%
  {\RstStateLineWidth%
   \RstStateLineStyle\RstStateLineColor%
   \RstStateBkgdStyle\RstStateBkgdColor%
   \RstStateLabelColor\RstStateLabelScale%
   \RstStateLabelSize\RstStateLabelStyle%
   \RstAsideLabelDirct\RstAsideLabelDistn%
  }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state label parameter computation}%%%%%
% extra space parameters
\newlength{\ExtraSpaceForCrcState}
\newlength{\ExtraSpaceForOvlState}
\newlength{\ExtraSpaceForRctState}
%
\newlength{\LabelBoxWidth}\newlength{\LabelBoxHeight}
\newcommand{\NulLabelBoxWidth}{\setlength{\LabelBoxWidth}{0pt}}
\newcommand{\NulLabelBoxHeight}{\setlength{\LabelBoxHeight}{0pt}}
%%%
% compose the label at the right scale, with the right size
% and in the right style
\newcommand{\SizedStateLabel}[1]%
    {\scalebox{\StateLabelSca}%
       {\scalebox{\StateLabelScale}%
	  {\StateLabelSz \SttLblMode\StateLabelSty{#1}\SttLblMode}}}
%%%
% compute the width of the composed label, 
% adjusted according to the shape of the state
\newcommand{\ComputLabelBoxWnH}[1]%
    {%
     \ifVCStateLabelInside%
        \settowidth{\LabelBoxWidth}{\SizedStateLabel{#1}}% width of lbl                  
        \settodepth{\VCSGTmpLength}{\SizedStateLabel{#1}}	
        \settoheight{\LabelBoxHeight}{\SizedStateLabel{#1}}%                  
        \addtolength{\LabelBoxHeight}{\VCSGTmpLength}%height of label
% add extra space, according to the shape
	\ifthenelse{\equal{\VCSttShp}{circle}}% 
           {\addtolength{\LabelBoxWidth}{\ExtraSpaceForCrcState}%
            \addtolength{\LabelBoxHeight}{\ExtraSpaceForCrcState}}%
            {\ifthenelse{\equal{\VCSttShp}{square}}%\or\equal{\VCSttShp}{rectangle}mystery
               {\addtolength{\LabelBoxWidth}{\ExtraSpaceForRctState}%
                \addtolength{\LabelBoxHeight}{\ExtraSpaceForRctState}}%
                {\ifthenelse{\equal{\VCSttShp}{rectangle}}%
                   {\addtolength{\LabelBoxWidth}{\ExtraSpaceForRctState}%
                    \addtolength{\LabelBoxHeight}{\ExtraSpaceForRctState}}%
                   {\ifthenelse{\equal{\VCSttShp}{oval}}% 
                      {\addtolength{\LabelBoxWidth}{\ExtraSpaceForOvlState}%
                       \addtolength{\LabelBoxHeight}{\ExtraSpaceForOvlState}}%
		      {ErrSttShape}%
                    }%
                 }%
	     }%
     \else% set size to 0
        \NulLabelBoxWidth\NulLabelBoxHeight%
     \fi
     }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% compute the shift for labels on baseline 
\newlength{\VertShiftH}\newlength{\VertShiftD}\newlength{\VertShift}%
\newcommand{\VCSFixVertShift}%
   {\settoheight{\VertShiftH}%
      {{\StateLabelSz \SttLblMode\StateLabelSty{\{}\SttLblMode}}%
    \settodepth{\VertShiftD}%
      {{\StateLabelSz \SttLblMode\StateLabelSty{\{}\SttLblMode}}%
    \setlength{\VertShift}{.5\VertShiftD-.5\VertShiftH}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% compute the distance for side labels 
\newlength{\AsdLblDst}%
\newcommand{\VCSFixAsdLblDst}%
   {\VCSGGreaterLgt{\LastSttDrawnWidth}{\LastSttDrawnHeight}{\VCSGTmpLength}%
    \CorrPosSttIntDim{\VCSGTmpLength}%
    \setlength{\AsdLblDst}{.5\VCSGTmpLength}%
    \addtolength{\AsdLblDst}{\AsideLabelDst}%
    }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state label writing}%%%%%
\newcommand{\WriteStateLabel}[2]%
    {\ifVCShowStt%
        \ifVCStateLabelInside%
           \rput#2{\makebox[0pt]{\WrtStateLabelIns{#1}}}%
        \else%
           \rput#2{\makebox[0pt]{\WrtStateLabelAsd{#1}}}%
        \fi%
     \fi}%
\newcommand{\WrtStateLabelIns}[1]%
    {\ifVCRigidStateLabel%
       \ifVCStateLabelOnBaseLine%
         {\VCSFixVertShift%
	  \textcolor{\StateLabelCol}%
	    {\scalebox{\StateLabelSca}%
               {\scalebox{\StateLabelScale}%
                  {\rput[B]{*0}(0,\VertShift){\WrtSttLbl{#1}}}}}}%
       \else
         {%
          \textcolor{\StateLabelCol}%
	     {\scalebox{\StateLabelSca}%
                {\scalebox{\StateLabelScale}%
                   {\rput{*0}(0,0){\WrtSttLbl{#1}}}}}}%
       \fi
     \else% TO BE FIXED  StateLabelOnBaseLine should be active
       {%
        \textcolor{\StateLabelCol}%
	  {\scalebox{\StateLabelSca}%
             {\scalebox{\StateLabelScale}%
                {\rput{0}(0,0){\WrtSttLbl{#1}}}}}}%
     \fi}
\newcommand{\WrtStateLabelAsd}[1]%
    {\VCSFixAsdLblDst%
     \ifVCRigidStateLabel%
        {\uput{\AsdLblDst}[\AsideLabelDir](0,0)%
           {\textcolor{\StateLabelCol}%
              {\scalebox{\StateLabelSca}%
                 {\scalebox{\StateLabelScale}%
                     {\WrtSttLbl{#1}}}}}}%
     \else% 
        {\uput{\AsdLblDst}[\AsideLabelDir](0,0)%
           {\textcolor{\StateLabelCol}%
              {\scalebox{\StateLabelSca}%
                 {\scalebox{\StateLabelScale}%
                    {\WrtSttLbl{#1}}}}}}%
     \fi}
\newcommand{\WrtSttLbl}[1]%
  {\StateLabelSz\SttLblMode\StateLabelSty{\VCLbl{#1}}\SttLblMode}%
% \newcommand{\VCLbl}[1]%
%    {\ifthenelse{\lengthtest{\LblBxLnWd = 0pt}}%
%       {#1}%
%       {\psframebox%
%           [doubleline=false,%
%            fillstyle=none,%
%            linestyle=solid,%
%            linecolor=\LblBxLnClr,%
%            linewidth=\LblBxLnWd,%
%            linearc=0pt,dimen=outer]%
%           {#1}}%
%     }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
\newcommand{\VCPutStateLabel}[2]{\rput#1{\WrtSttLbl{#2}}}
\newcommand{\AsideStateLabel}[2]%
    {\SpecialCoor%
     \rput(#1){\makebox[0pt]{\WrtStateLabelAsd{#2}}}%
     \NormalCoor%
     }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{construction lines}%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% construction line parameter
\newcommand{\SqrSttCtrClr}{}
\newcommand{\LblBxLnClr}{}
\newcommand{\PhtSttLnClr}{}
\newlength{\SqrSttCtr}
\newlength{\LblBxLnWd}
\newlength{\PhtSttLnWd}
\newlength{\PhtSttCtr}
\newlength{\PhtSttInt}
% construction line commands
\newcommand{\CtrBxLblOn}{\setlength{\LblBxLnWd}{0.3pt}}
\newcommand{\CtrBxLblOff}{\setlength{\LblBxLnWd}{0pt}}
\newcommand{\CtrSqrSttOn}{\setlength{\SqrSttCtr}{0.3pt}}
\newcommand{\CtrSqrSttOff}{\setlength{\SqrSttCtr}{0pt}}
\newcommand{\CtrPhtSttOn}{\setlength{\PhtSttLnWd}{0.3pt}}
\newcommand{\CtrPhtSttOff}{\setlength{\PhtSttLnWd}{0pt}}
% construction line functions
% Draw a box around the parameter (originaly a label, hence the name) 
% when the length \LblBxLnWd has been given a value different from 0 
\newcommand{\VCLbl}[1]%
   {\ifthenelse{\lengthtest{\LblBxLnWd = 0pt}}%
      {#1}%
      {\psframebox%
          [doubleline=false,%
           fillstyle=none,%
           linestyle=solid,%
           linecolor=\LblBxLnClr,%
           linewidth=\LblBxLnWd,%
           linearc=0pt,dimen=outer]%
          {#1}}%
    }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{internal state parameters}%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% internal parameters
\newlength{\SttIntDiamtr}
\newlength{\SttIntWidth}
\newlength{\SttIntHeight}
\newlength{\OvlSttIntWidth}
\newlength{\OvlSttIntHeight}
\newlength{\StateVarWidth}
% twice the distance between the center of state
% and the centers of the phantom states 
\newlength{\SttVarWidthShift}
\newlength{\SttVarHeightShift}
%%%
\newlength{\ActiveLineWidth}
\newcommand{\ActiveDimen}{}
\newcommand{\CorrNegSttIntDim}[1]%
    {\ifStateLineDbl%
        \renewcommand{\ActiveDimen}{\SttDblLineDimen}%
	\setlength{\ActiveLineWidth}{\SttLineDblCoef\StateLineWid}%
	\addtolength{\ActiveLineWidth}{\SttLineDblCoef\StateLineWid}%
	\addtolength{\ActiveLineWidth}{\SttLineDblSep\StateLineWid}%
     \else%
        \renewcommand{\ActiveDimen}{\SttDimen}%
	\setlength{\ActiveLineWidth}{\StateLineWid}%
     \fi%
     \ifthenelse{\equal{\ActiveDimen}{outer}}%
        {\addtolength{#1}{-2\StateLineWid}}%
        {\ifthenelse{\equal{\ActiveDimen}{middle}}%
            {\addtolength{#1}{-\StateLineWid}}%
            {}%
	 }%
    }
\newcommand{\CorrPosSttIntDim}[1]%
    {\ifStateLineDbl%
        \renewcommand{\ActiveDimen}{\SttDblLineDimen}%
        \setlength{\ActiveLineWidth}{\SttLineDblCoef\StateLineWid}%
        \addtolength{\ActiveLineWidth}{\SttLineDblCoef\StateLineWid}%
        \addtolength{\ActiveLineWidth}{\SttLineDblSep\StateLineWid}%
     \else%
        \renewcommand{\ActiveDimen}{\SttDimen}%
        \setlength{\ActiveLineWidth}{\StateLineWid}%
     \fi%
     \ifthenelse{\equal{\ActiveDimen}{outer}}%
        {\addtolength{#1}{2\StateLineWid}}%
        {\ifthenelse{\equal{\ActiveDimen}{middle}}%
            {\addtolength{#1}{\StateLineWid}}%
            {}%
         }%
    }
%%%
\newcommand{\ComputSttIntDimension}%
    {%
     \setlength{\SttIntWidth}{\StateDia}%
     \setlength{\SttIntHeight}{\StateDia}%
     \setlength{\PhtSttInt}{\StateDia}%
     \addtolength{\PhtSttInt}{-2\PhtSttLnWd}
     \ifthenelse{\equal{\VCSttShp}{circle}\or\equal{\VCSttShp}{square}}%
       {}% do nothing
%        {\ifthenelse{\equal{\VCSttShp}{square}}%
%          {}% do nothing
	 {\ifthenelse{\equal{\VCSttShp}{rectangle}}%
	   {\ifthenelse{\VCSGCmdPosTst{\RectangleStateRat}}%
	     {\setlength{\SttIntWidth}{\RectangleStateRat\StateDia}}%
             {\setlength{\SttIntHeight}{\RectangleStateRat\StateDia}%
              \setlength{\SttIntHeight}{-\SttIntHeight}}%
	   }%
	   {\ifthenelse{\equal{\VCSttShp}{oval}}%
	     {\ifthenelse{\VCSGCmdPosTst{\OvalStateRat}}%
	       {\setlength{\SttIntWidth}{\OvalStateRat\StateDia}}%
               {\setlength{\SttIntHeight}{\OvalStateRat\StateDia}%
		\setlength{\SttIntHeight}{-\SttIntHeight}}%
             }%
	     {ErrSttShape}%
           }%
%          }%
       }%
     \CorrNegSttIntDim{\SttIntWidth}%
     \CorrNegSttIntDim{\SttIntHeight}%
    }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{Internal state drawing commands}%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\IntCrossTmp}%
\newcommand{\IntCross}[3]%
   {\setlength{\IntCrossTmp}{#1}\addtolength{\IntCrossTmp}{-#3}%
    {\color{\SqrSttCtrClr}%
     {\protect\rule[-.5#3]{.5\IntCrossTmp}{#3}%
     \protect\rule[-.5#2]{#3}{#2}%
     \protect\rule[-.5#3]{.5\IntCrossTmp}{#3}}%
    }}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% defines and draws a circle state
\newcommand{\VCSGCrcState}[3]{\rput#1{\Cnode[radius=.5#3](0,0){#2}}}
% defines and draws a square state
\newcommand{\VCSGSqrState}[4]%
   {\rput#1{\rnode{#2}{\psframebox{\IntCross{#3}{#4}{\SqrSttCtr}}}}}
% defines and draws an oval state
\newcommand{\VCSGOvlState}[4]%
   {\setlength{\OvlSttIntWidth}{\HSQRTwo#3}%
    \setlength{\OvlSttIntHeight}{\HSQRTwo#4}%
    \rput#1{\ovalnode{#2}%
               {\IntCross{\OvlSttIntWidth}{\OvlSttIntHeight}{\SqrSttCtr}}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% call for the drawing of a state of normal size
\newcommand{\DrawState}[2]%
   {\SttStyle%
    \ifthenelse{\equal{\VCSttShp}{circle}}%
       {\VCSGCrcState{#1}{#2}{\StateDia}}%
       {\ifthenelse{\equal{\VCSttShp}{square}\or\equal{\VCSttShp}{rectangle}}%
           {\VCSGSqrState{#1}{#2}{\SttIntWidth}{\SttIntHeight}}%
           {\ifthenelse{\equal{\VCSttShp}{oval}}%
               {\VCSGOvlState{#1}{#2}{\SttIntWidth}{\SttIntHeight}}%
               {ErrorStateShape \VCSttShp}%
            }%
        }%
    }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ProcessState}[3]%
   {%
    \RazSttVar
    \ifVCSizedNode%
 	\ProcessSizedState{#1}{#2}{#3}%   
    \else
 	\ProcessSizelessState{#1}{#2}{#3}%   
    \fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\State}[3][{}]%
   {\renewcommand{\VCSttShp}{\VCSttShape}\ProcessState{#1}{#2}{#3}}  
\newcommand{\CrcState}[3][{}]%
   {\renewcommand{\VCSttShp}{circle}\ProcessState{#1}{#2}{#3}}   
\newcommand{\OvlState}[3][{}]%
   {\renewcommand{\VCSttShp}{oval}\ProcessState{#1}{#2}{#3}}   
\newcommand{\SqrState}[3][{}]%
   {\renewcommand{\VCSttShp}{square}\ProcessState{#1}{#2}{#3}}   
\newcommand{\RctState}[3][{}]%
   {\renewcommand{\VCSttShp}{rectangle}\ProcessState{#1}{#2}{#3}}   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{variable states}%%
%%%
%  A flag for the variable state plolicy:
%    true:  size of label control whether state is "Var" or not
%    false: state is "Var" only when declared so
\newif\ifAdjstSttFlg 
\newcommand{\SelfAdjustState}{\AdjstSttFlgtrue}
\newcommand{\FixedSizeState}{\AdjstSttFlgfalse}
%  Mode of variable states
\newcommand{\VCSttVarMode}{}
% horizontal, vertical (Two phantom states created) 
% total        (Four phantom states created)
% hypertotal   (Eight phantom states created) -- not implemented
% homothetic   (No phantom states created)
\newcommand{\HorizontalStateVarMode}{\renewcommand{\VCSttVarMode}{horizontal}}
\newcommand{\VerticalStateVarMode}{\renewcommand{\VCSttVarMode}{vertical}}
\newcommand{\TotalStateVarMode}{\renewcommand{\VCSttVarMode}{total}}
\newcommand{\HomotheticStateVarMode}{\renewcommand{\VCSttVarMode}{homothetic}}
%
\newcommand{\StateVarMode}[1]{\renewcommand{\VCSttVarMode}{#1}}
%%%
%  Flags to remember if the last state drawn is a variable state
%  commands are for internal use
\newif\ifVCSttVar  
\newif\ifVCSttVarH  
\newif\ifVCSttVarV  
\newcommand{\RazSttVar}%
   {\VCSttVarfalse\VCSttVarHfalse\VCSttVarVfalse}
\newcommand{\IsSttVar}{\VCSttVartrue}
\newcommand{\IsSttVarH}{\VCSttVarHtrue}
\newcommand{\IsSttVarV}{\VCSttVarVtrue}
\RazSttVar % initialization, as it is internal 
%%%
% In case of Circle State, variable states are made by rectangle,
% with corner rounded with a radius equal to the half of the height.
\newpsstyle{CrcStateVarStyle}%
        {%
         cornersize=absolute,%
	 linearc=0.5\StateDia}%
%%% syle for the phantom states
\newpsstyle{NoPhtStateStyle}%
        {framesep=0pt,%
         fillstyle=none,%
         linewidth=\PhtSttLnWd,%
         linestyle=none,%
         linecolor=green,%
         doubleline=false,%
         dimen=outer}%
\newpsstyle{PhtStateStyle}%
        {framesep=0pt,%
         fillstyle=none,%
         linewidth=\PhtSttLnWd,%
         linestyle=dashed,%
         linecolor=\PhtSttLnClr,%
         doubleline=false,%
         dimen=outer}%
%%%
\newcommand{\CrcSttVarStyle}%
   {\ifVCShowStt\psset{style=CrcStateVarStyle}%
        \else\psset{style=VCHiddenStateStyle}\fi}
\newcommand{\PhtSttVarStyle}%
   {\ifVCShowStt%
       \ifthenelse{\lengthtest{\PhtSttLnWd = 0pt}}%
           {\psset{style=NoPhtStateStyle}}%
           {\psset{style=PhtStateStyle}}%
        \else\psset{style=VCHiddenStateStyle}\fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% call for the drawing of a state of variable size
%%% Choice between the var modes
\newcommand{\DrawStateVar}[2]% 
   {\SttStyle%
    \ifthenelse{\equal{\VCSttVarMode}{horizontal}}%
       {\ifVCSttVarH\DrawStateVarH{#1}{#2}\else\DrawState{#1}{#2}\fi}%
       {\ifthenelse{\equal{\VCSttVarMode}{vertical}}%
           {\ifVCSttVarV\DrawStateVarV{#1}{#2}\else\DrawState{#1}{#2}\fi}%
           {\ifthenelse{\equal{\VCSttVarMode}{total}}%
               {\DrawStateVarT{#1}{#2}}%
               {\ifthenelse{\equal{\VCSttVarMode}{homothetic}}%
                   {\DrawStateVarM{#1}{#2}}%
                   {ErrorStateVarMode \VCSttVarMode}%
               }%
           }%
       }%
   }%
%%% Square phantom state
\newcommand{\SqrPhtStt}{\psframebox{\IntCross{\PhtSttInt}{\PhtSttInt}{\PhtSttCtr}}}
%%% Choice between the shapes
\newcommand{\DrawStateVarH}[2]%
   {\SttStyle%
    \setlength{\SttVarWidthShift}{\LastSttDrawnWidth}%
    \addtolength{\SttVarWidthShift}{-\StateDia}% 
    \CorrPosSttIntDim{\SttVarWidthShift}% 
    \ifthenelse{\equal{\VCSttShp}{circle}}%
       {\CrcSttVarStyle%
        \VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}%
        \PhtSttVarStyle%
        \rput#1{\Cnode[radius=.5\StateDia](.5\SttVarWidthShift,0){#2e}}%
        \rput#1{\Cnode[radius=.5\StateDia](-.5\SttVarWidthShift,0){#2w}}%
        }%
       {\ifthenelse{\equal{\VCSttShp}{square}\or\equal{\VCSttShp}{rectangle}}%
           {\VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}%
            \PhtSttVarStyle%
            \rput#1{\rput(.5\SttVarWidthShift,0){\rnode{#2e}{\SqrPhtStt}}}%
            \rput#1{\rput(-.5\SttVarWidthShift,0){\rnode{#2w}{\SqrPhtStt}}}%
            }%
           {\ifthenelse{\equal{\VCSttShp}{oval}}%
                {\VCSGOvlState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}}%
                {ErrorStateShape \VCSttShp}%
            }%
       }%
   }%
%%% Choice between the shapes
\newcommand{\DrawStateVarV}[2]%
   {\SttStyle%
    \setlength{\SttVarHeightShift}{\LastSttDrawnHeight}%
    \addtolength{\SttVarHeightShift}{-\StateDia}% 
    \CorrPosSttIntDim{\SttVarHeightShift}% 
    \ifthenelse{\equal{\VCSttShp}{circle}}%
       {\CrcSttVarStyle%
        \VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}%
        \PhtSttVarStyle%
        \rput#1{\Cnode[radius=.5\StateDia](0,.5\SttVarHeightShift){#2n}}%
        \rput#1{\Cnode[radius=.5\StateDia](0,-.5\SttVarHeightShift){#2s}}%
        }%
       {\ifthenelse{\equal{\VCSttShp}{square}\or\equal{\VCSttShp}{rectangle}}%
           {\VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}%
            \PhtSttVarStyle%
            \rput#1{\rput(0,.5\SttVarHeightShift){\rnode{#2n}{\SqrPhtStt}}}%
            \rput#1{\rput(0,-.5\SttVarHeightShift){\rnode{#2s}{\SqrPhtStt}}}%
            }%
           {\ifthenelse{\equal{\VCSttShp}{oval}}%
                {\VCSGOvlState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}}%
                {ErrorStateShape \VCSttShp}%
            }%
       }%
   }%
%%% Choice between the shapes
\newcommand{\DrawStateVarT}[2]%
   {\SttStyle%
    \setlength{\SttVarWidthShift}{\LastSttDrawnWidth}%
    \addtolength{\SttVarWidthShift}{-\StateDia}% 
    \CorrPosSttIntDim{\SttVarWidthShift}% 
    \setlength{\SttVarHeightShift}{\LastSttDrawnHeight}%
    \addtolength{\SttVarHeightShift}{-\StateDia}% 
    \CorrPosSttIntDim{\SttVarHeightShift}% 
    \ifthenelse{\equal{\VCSttShp}{circle}}%
       {\CrcSttVarStyle%
        \VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}%
        \SttStyle\PhtSttVarStyle%
        \rput#1{\rput(.5\SttVarWidthShift,0){\rnode{#2e}{\SqrPhtStt}}}%
        \rput#1{\rput(-.5\SttVarWidthShift,0){\rnode{#2w}{\SqrPhtStt}}}%
        \rput#1{\rput(0,.5\SttVarHeightShift){\rnode{#2n}{\SqrPhtStt}}}%
        \rput#1{\rput(0,-.5\SttVarHeightShift){\rnode{#2s}{\SqrPhtStt}}}%
        }%
       {\ifthenelse{\equal{\VCSttShp}{square}\or\equal{\VCSttShp}{rectangle}}%
           {\VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}%
            \PhtSttVarStyle%
            \rput#1{\rput(.5\SttVarWidthShift,0){\rnode{#2e}{\SqrPhtStt}}}%
            \rput#1{\rput(-.5\SttVarWidthShift,0){\rnode{#2w}{\SqrPhtStt}}}%
            \rput#1{\rput(0,.5\SttVarHeightShift){\rnode{#2n}{\SqrPhtStt}}}%
            \rput#1{\rput(0,-.5\SttVarHeightShift){\rnode{#2s}{\SqrPhtStt}}}%
            }%
            {\ifthenelse{\equal{\VCSttShp}{oval}}%
                {\VCSGOvlState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}}%
                {ErrorStateShape \VCSttShp}%
             }%
        }%
    }%
%%% Choice between the shapes
\newcommand{\DrawStateVarM}[2]%
   {\SttStyle%
    \ifthenelse{\equal{\VCSttShp}{circle}}%
       {\VCSGGreaterLgt{\LastSttDrawnWidth}{\LastSttDrawnHeight}{\VCSGTmpLength}%
        \VCSGCrcState{#1}{#2}{\VCSGTmpLength}}%
       {\ifthenelse{\equal{\VCSttShp}{square}}%
           {\VCSGGreaterLgt{\LastSttDrawnWidth}{\LastSttDrawnHeight}{\VCSGTmpLength}%
            \VCSGSqrState{#1}{#2}{\VCSGTmpLength}{\VCSGTmpLength}}%%
           {\ifthenelse{\equal{\VCSttShp}{rectangle}}%
               {\ifthenelse{\VCSGCmdPosTst{\RectangleStateRat}}%
                   {\setlength{\VCSGTmpLength}{\RectangleStateRat\LastSttDrawnHeight}%
                    \ifthenelse{\lengthtest{\VCSGTmpLength>\LastSttDrawnWidth}%
                                \or\lengthtest{\VCSGTmpLength=\LastSttDrawnWidth}}%
                        {\VCSGSqrState{#1}{#2}{\VCSGTmpLength}{\LastSttDrawnHeight}}%
                        {\setlength{\VCSGTmpLength}{\LastSttDrawnWidth*\ratio{1pt}{\RectangleStateRat pt}}%
                         \VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\VCSGTmpLength}}%%
                    }%    
                   {\setlength{\VCSGTmpLength}{-\RectangleStateRat\LastSttDrawnWidth}%
                    \ifthenelse{\lengthtest{\VCSGTmpLength>\LastSttDrawnHeight}%
                                \or\lengthtest{\VCSGTmpLength=\LastSttDrawnHeight}}%
                        {\VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\VCSGTmpLength}}%%
                        {\setlength{\VCSGTmpLength}{\LastSttDrawnHeight*\ratio{1pt}{-\RectangleStateRat pt}}%
                         \VCSGSqrState{#1}{#2}{\VCSGTmpLength}{\LastSttDrawnHeight}}%%
                    }%
                }%
               {\ifthenelse{\equal{\VCSttShp}{oval}}%
                   {\ifthenelse{\VCSGCmdPosTst{\OvalStateRat}}%
                       {\setlength{\VCSGTmpLength}{\OvalStateRat\LastSttDrawnHeight}%
                        \ifthenelse{\lengthtest{\VCSGTmpLength>\LastSttDrawnWidth}%
                                    \or\lengthtest{\VCSGTmpLength=\LastSttDrawnWidth}}%
                           {\setlength{\OvlSttIntWidth}{\HSQRTwo\VCSGTmpLength}%
                            \setlength{\OvlSttIntHeight}{\HSQRTwo\LastSttDrawnHeight}}%
                           {\setlength{\VCSGTmpLength}{\LastSttDrawnWidth*\ratio{1pt}{\OvalStateRat pt}}%
                            \setlength{\OvlSttIntWidth}{\HSQRTwo\LastSttDrawnWidth}%
                            \setlength{\OvlSttIntHeight}{\HSQRTwo\VCSGTmpLength}}}%    
                       {\setlength{\VCSGTmpLength}{-\OvalStateRat\LastSttDrawnWidth}%
                        \ifthenelse{\lengthtest{\VCSGTmpLength>\LastSttDrawnHeight}%
                                    \or\lengthtest{\VCSGTmpLength=\LastSttDrawnHeight}}%
                           {\setlength{\OvlSttIntWidth}{\HSQRTwo\LastSttDrawnWidth}%
                            \setlength{\OvlSttIntHeight}{\HSQRTwo\VCSGTmpLength}}%
                           {\setlength{\VCSGTmpLength}{\LastSttDrawnHeight*\ratio{1pt}{-\OvalStateRat pt}}%
                            \setlength{\OvlSttIntWidth}{\HSQRTwo\VCSGTmpLength}%
                            \setlength{\OvlSttIntHeight}{\HSQRTwo\LastSttDrawnHeight}}}%
                    \rput#1{\ovalnode{#2}{\IntCross{\OvlSttIntWidth}{\OvlSttIntHeight}{\SqrSttCtr}}}%
                    }%
                   {ErrorStateShape \VCSttShp}%
                }%
            }%
        }%
    }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% record the width, and the height, of the composed label
% and whether it makes the state a "variable" one.
\newlength{\LastSttDrawnHeight}
\newlength{\LastSttDrawnWidth}
\newcommand{\FixVarSttDrawingPar}%
    {%
     \RazSttVar%
     \ifthenelse{\lengthtest{\LabelBoxWidth > \SttIntWidth}%
                 \and\(\not\equal{\VCSttVarMode}{vertical}\)}%
        {\IsSttVarH\IsSttVar%
         \setlength{\LastSttDrawnWidth}{\LabelBoxWidth}}%
        {\setlength{\LastSttDrawnWidth}{\SttIntWidth}}%
     \ifthenelse{\lengthtest{\LabelBoxHeight > \SttIntHeight}%
                 \and\(\not\equal{\VCSttVarMode}{horizontal}\)}%
        {\IsSttVarV\IsSttVar%
         \setlength{\LastSttDrawnHeight}{\LabelBoxHeight}}%
        {\setlength{\LastSttDrawnHeight}{\SttIntHeight}}%
    }%
%%%%%\section{process states}%%%%%%%%%%%%%%%%%%%
% the top calling procedure for drawing states
% when entering that procedure, 
% \VCSttShp should be given the right value
\newcommand{\ProcessSizedState}[3]%
    {\ComputSttIntDimension%
     \ComputLabelBoxWnH{#1}%
     \ifAdjstSttFlg 
     \else 
        \NulLabelBoxWidth\NulLabelBoxHeight%
     \fi% 
     \FixVarSttDrawingPar%
     \ifVCSttVar
        \DrawStateVar{#2}{#3}%
     \else
        \DrawState{#2}{#3}%
     \fi%
     \WriteStateLabel{#1}{#2}%
    }%
%%% the same, without the test on AdjstSttFlg
\newcommand{\ProcessSizedStateVar}[3]%
    {\ComputSttIntDimension%
     \ComputLabelBoxWnH{#1}%
     \FixVarSttDrawingPar%
      \ifVCSttVar
         \DrawStateVar{#2}{#3}%
      \else
         \DrawState{#2}{#3}%
      \fi%
     \WriteStateLabel{#1}{#2}%
    }
%%%
\newcommand{\StateVar}[3][{}]%
   {\renewcommand{\VCSttShp}{\VCSttShape}
    \RazSttVar%
    \ifVCSizedNode%
 	\ProcessSizedStateVar{#1}{#2}{#3}%   
    \else
 	\ProcessSizelessState{#1}{#2}{#3}%   
    \fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newcommand{\FinalSttStyle}%
   {\ifVCShowStt\psset{style=VcsnStateDblStyle}%
    \else\psset{style=VcsnHiddenStateStyle}\fi}
\newcommand{\DotSttStyle}%
   {\ifVCShowStt\psset{style=VcsnVertexStyle}%
        \else\psset{style=VcsnHiddenStateStyle}\fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%\section{backward compatibility}%%%%%%
%%%%%  Obsolete commands from version 0.3, 0.4 and 1.0
%%%%%  kept for backward compatibility
%%%%%  cf users manual for description of compatibilty problems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\StateDimen}{}
\newcommand{\StateDblDimen}{}
%
\newcommand{\SetStateFillColor}[1]{\SetStateBkgdColor{#1}}%
\newcommand{\SetStateFillStatus}[1]{\SetStateBkgdStyle{#1}}%
\newcommand{\SmallStateFillColor}{}% apparently not used in 0.4 either
%% state size
\newcommand{\MediumState}{\MediumStates}
\newcommand{\SmallState}{\SmallStates}
\newcommand{\LargeState}{\LargeStates}
%%% hiding--showing
\newcommand{\HideState}{\HideStates}
\newcommand{\ShowState}{\ShowStates}
%%% hiding--showing
\newcommand{\AlignedLabel}{\AlignedStateLabel}
\newcommand{\FloatingLabel}{\FloatingStateLabel}
%%% dim states 
%%% (tricky compatibility: order of parameters has changed!)
\newcommand{\FixDimState}[5]{\SetDimStatePmts{#1}{#3}{#2}{#4}{#5}} 
%%% ecological commands (obsolete from v. 1.0 on -- idem state) 
\newcommand{\StateIF}[3][{}]{\State[#1]{#2}{#3}}%
\newcommand{\StateIFX}[3][{}]{\State[#1]{#2}{#3}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Very Small State   
\newcommand{\VSStateLineCoef}{.6} % coef. for very small state
\newcommand{\VSState}[2]%
    {\renewcommand{\ArrowOnStateCoef}{\ArrowOnVerySmallState}%
     \FixStateDiameter{\VerySmallStateDiameter}%
     \ChgStateLineWidth{\VSStateLineCoef}%
         \State{#1}{#2}%
         \RstStateLineWidth\RstSttDiameter}% mod 020201
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\RigidLabel}{\VCRigidStateLabeltrue}
\newcommand{\SwivelLabel}{\VCRigidStateLabelfalse}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % changing/setting the width of state border 
% %        (the space between state line and the transitions) NON!
% \newcommand{\ChgStateBorderWidth}[1]%
%    {\setlength{\StateBorderWid}{#1\StateBorderWidth}}  
% \newcommand{\RstStateBorderWidth}{\ChgStateBorderWidth{1}}
% \newcommand{\SetStateBorderWidth}[1]% ATTN the parameter is a length
%    {\setlength{\StateBorderWidth}{#1}\RstStateBorderWidth}


==> VCSGPref-beamer.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Package `VauCanSon-G'  version 0.4
%%
%% This is file `VCPref-slides'.
%%
%% IMPORTANT NOTICE:
%%
%% Copyright (C) 2002-2008 Sylvain Lombardy and Jacques Sakarovitch
%%
%% This package may be distributed under the terms of the LaTeX Project
%% Public License, as described in lppl.txt in the base LaTeX distribution.
%% Either version 1.0 or, at your option, any later version.
%%
%% DESCRIPTION:
%%
%%   `VCPref-beamer' contains initial values of VauCanSon-G 
%%   parameters suitable for drawing automata in slides.
%%   Works with package `beamer'; 
%%   smaller scale values than those given in `VCPref-slides'
%%  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scales  --- slides settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\LargeScale}{0.85}       
\renewcommand{\MediumScale}{0.6}       
\renewcommand{\SmallScale}{0.4}		
\renewcommand{\TinyScale}{0.30}		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% State aspect
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetStateLineWidth{2pt}
\SetStateLineColor{blue}
\SetStateBkgdColor{Cyan}
\SetStateLabelColor{Sepia}
%%% Dimmed states
\SetDimStatePmts{solid}{1}{YellowOrange}{YellowOrange}{white}
%%%%%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetEdgeLineColor{Mahogany}
\SetEdgeLineWidth{1.2pt}
\SetEdgeLabelColor{OliveGreen}
%%% Dimmed edges
\SetDimEdgePmts{dashed}{1.2}{Apricot}{Apricot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initialization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\HideFrame
\HideGrid
\HideName
\MediumState
\MediumPicture
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput


==> VCSGPref-mystyle.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:    VCPref-mystyle
%%
%% DESCRIPTION:  personal setting of VauCanSon-G's parameters
%%
%  By definiton, an empty file to be customised.
%  
%  VCSG-Preferences.tex is copied after the \endinput
%  andcan be used as a template to write 
%  a customized style of Vaucanson.
%  
%%  
%% DATE:    2012/07/05
%%
%% Copyright (C) 2009-2012 Sylvain Lombardy and Jacques Sakarovitch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-environment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Scaling matters}%%%%%  
% Inner parameters
\renewcommand{\LargeScale}{0.85}    %float : argument of a \scalebox
\renewcommand{\LargeScaleI}{1.18}
\renewcommand{\MediumScale}{0.6}    %float
\renewcommand{\MediumScaleI}{1.67}
\renewcommand{\SmallScale}{0.5}     %float
\renewcommand{\SmallScaleI}{2}
\renewcommand{\TinyScale}{0.42}     %float
\renewcommand{\TinyScaleI}{2.38}
%
\MediumPictures
\FixVCGridScale{1}
%%%%%\section{Picture directory}%%%%%
% \SetVCDirectory{}  % for record : the definition of \VCDirectory is 
%                    % an initialisation 
%%%%%\section{Picture framing}%%%%%
% Inner parameters
\setlength{\VCFrameLineWidth}{0.6pt}
\renewcommand{\VCFrameLineColor}{black}
\setlength{\VCGridLineWidth}{0.6pt}
\renewcommand{\VCGridLineColor}{black}
%
\SetVCBkgdStyle{solid} % Also set StateBkgd, SmallStateBkgd,
                       % SttBorderColor,EdgeLineBorderColor
\SetVCBkgdColor{white} % and DblEdgeLineColor
%
\HideFrame\HideGrid\HideName
%%%%%\section{Picture drawing call}%%%%%
\FixVerticalPlacement{0.5} %float 
%%%%%\section{VauCanSon-G modes}%%%%%
\Automata 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-states}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{node mode}%%%%%%
% \SizedNodes % for record; not necessary after the call to \Automata 
%%%%%\section{state size}%%%%%%
\setlength{\SmallStateDiameter}{.6cm}
\setlength{\MediumStateDiameter}{1cm}
\setlength{\LargeStateDiameter}{1.2cm}
% \FixStateSizes{.6cm}{.9cm}{1.2cm}{.3cm} would have the same effect
%
% \MediumStates postponed after the definition of loop geometry 
% parameters
%%%%%\section{state shape}%%%%%
\CircleStates
\SetOvalStateRatio{\GoldMeanI}
\SetRectangleStateRatio{\GoldMeanI}
%
\SharpStateCorners 
\StateCornerRoundingAbsolute
\SetStateCornerRelRadius{0}
\SetStateCornerRadius{0.2cm}
%%%%%\section{Hiding -- showing}%%%%%
\ShowStates
%%%%%\section{state background parameters}%%%%%
% for record: setting done when setting the Bkgd of the picture 
% \SetStateBkgdStyle{\VCBkgdStyle}\SetStateBkgdColor{\VCBkgdColor}
% \SetSmallStateBkgdStyle{\VCBkgdStyle}
% \SetSmallStateBkgdColor{\VCBkgdColor}
%%%%%\section{construction line parameters}%%%%%%
\renewcommand{\SqrSttCtrClr}{blue}
\renewcommand{\LblBxLnClr}{red}
\renewcommand{\PhtSttLnClr}{green}
\CtrBxLblOff
\CtrSqrSttOff
\CtrPhtSttOff
\setlength{\PhtSttCtr}{0pt} %%% 
%%%%%\section{state line parameters}%%%%%%
% Inner parameters
\renewcommand{\SttDimen}{outer}
\renewcommand{\SttDblLineDimen}{middle}
\setlength{\SttBorderWidth}{0pt}
% \renewcommand{\SttBorderColor}{\StateBkgdColor} for record
\FixStateLineDouble{0.6}{0.4}  
%%%%%\section{state line parameters}%%%%%%
\SetStateLineWidth{1.8pt}
\SetStateLineStyle{solid}
\SetStateLineColor{black}
%
\StateLineSimple
%%%%%\section{state label parameters}%%%%%
\RigidStateLabel\FloatingStateLabel\StateLabelInside
\SetStateLabelColor{black}
% \SetStateLabelScale{1.667} (set by the scale picture commands)
\SetStateLabelSize{\normalsize}
\StateLabelModeMath
\SetStateLabelStyle{}
\SetAsideLabelDirct{72}
\SetAsideLabelDistn{6pt}
%%% Variable States
% extra space between the label and the state line (to be fixed)
\setlength{\ExtraSpaceForCrcState}{4mm}
\setlength{\ExtraSpaceForOvlState}{2mm}
\setlength{\ExtraSpaceForRctState}{2mm}
% mode initialisation
\HorizontalStateVarMode\SelfAdjustState
%%% Sizeless States
\setlength{\VerySmallStateDiameter}{.3cm}
%%% Dimmed states
% \renewcommand{\DimStateLineStyle}{solid} 
% \renewcommand{\DimStateLineCoef}{1} % 
% \renewcommand{\DimStateLineColor}{gray}
% \renewcommand{\DimStateLabelColor}{gray}
% \renewcommand{\DimStateBkgdColor}{white}
\SetDimStatePmts{solid}{1}{gray}{gray}{white}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-edges}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge label drawing macros
\renewcommand{\InOutLbl}[2]{#1\!\mid\! #2} % other ex: {(#1, #2)} 
\renewcommand{\IOL}[2]{#1\!\mid\! #2} % downward compatibility 
\renewcommand{\LblCnnct}{+}
%%% Edge drawing parameters
%%% Line
\SetEdgeLineWidth{1pt}			%% width (length param.)
\SetEdgeLineStyle{solid}		%% aspect
\SetEdgeLineColor{black}		%% color
\EdgeLineSimple
% double line the two coefficients have already been initialised in 
% VCSG-edges.tex in order to avoid deadlock; the call to 
% \FixEdgeLineDouble completes the initialisation
\FixEdgeLineDouble{0.5}{0.6}		%% float : coefs*\EdgeLineWidth -> (width of lines, distance)
\SetDblEdgeLineColor{\VCBkgdColor} %% useless since it has 
              %% already been initialised with the picture background
% border
\EdgeLineBorderOff
\FixEdgeLineBorder{2}{\VCBkgdColor}		%% int,color : coef*\EdgeLineWidth -> width of border
%%% Edge arrow
\ArrowEdge				%% fix the style of arrows
% arrows on simple line 
\SetEdgeArrowWidthBase{2.5pt}
\SetEdgeArrowWidthCoef{2}
\SetEdgeArrowLengthCoef{1.4}
\SetEdgeArrowInsetCoef{0.1}
% idem  \SetEdgeArrowDimensions{2pt}{3}{1.4}{0.1}  
% arrows on double line 
\SetDblEdgeArrowWidthBase{2.5pt}
\SetDblEdgeArrowWidthCoef{1.6}
\SetDblEdgeArrowLengthCoef{1.3}
\SetDblEdgeArrowInsetCoef{0.1}
% idem  \SetDblEdgeArrowDimensions{2pt}{3}{1.4}{0.1}  
%%% Edge geometry parameters
\SetEdgeOffset{3pt}
\SetEdgeOffsetCoef{3}
\EdgeOffsetOff
\EdgeOffsetAbs
\SetForthBackEdgeOffsetCoef{2}% coef
\ForthBackOffsetOff
%
\NodeSeparationOff
\SetNodeSep{3pt}
%%% Edge label parameters
\EdgeLabelModeMath
\SetEdgeLabelSize{\normalsize}
\SetEdgeLabelStyle{}
\SetEdgeLabelColor{black}
\SetEdgeLabelScale{1.667}
%%% Edge label boxing parameters
\BoxedEdgeLabelOff
\renewcommand{\BxdEdgLblSep}{5}
\renewcommand{\BxdEdgLblBkg}{white}
\renewcommand{\BxdEdgLblWdt}{1}
\renewcommand{\BxdEdgLblStl}{solid}
\renewcommand{\BxdEdgLblCol}{black}
\renewcommand{\BxdEdgLblDbl}{false}
\renewcommand{\BxdEdgLblRnd}{0}
%%% Edge label geometry parameters
\DirectTransitions
\SetEdgLblPosit{.45}{.55}
\SetArcLblPosit{.4}{.6}
\SetLArcLblPosit{.4}{.6}
\SetLoopLblPosit{.25}{.75}
\SetCLoopLblPosit{.25}{.75}
%
\SetTransLabelSep{8pt}
%
\SwivelEdgeLabel
%%% Dimmed edges
% \renewcommand{\DimEdgeLineStyle}{solid} 
% \renewcommand{\DimEdgeLineCoef}{1.2} 
% \renewcommand{\DimEdgeLineColor}{gray}
% \renewcommand{\DimEdgeLabelColor}{gray}
\SetDimEdgePmts{solid}{1.2}{gray}{gray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Initial-final arrow drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\ArrowOnSmallState}{1.2} 		%float
\renewcommand{\ArrowOnMediumState}{1}		%float : coef *\StateDiameter for size of initial and final arrows
\renewcommand{\ArrowOnLargeState}{.8}		%float
% implicit parameter
\renewcommand{\InitialDir}{w}
\renewcommand{\FinalDir}{e}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Arc geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Angle
\SetArcAngle{15}
\SetLArcAngle{30}
% Curvature
\SetArcCurvature{0.8}
\SetLArcCurvature{0.8}
% Offset
\SetArcOffset{1pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Loop geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Angle
\SetLoopAngle{30}
\SetCLoopAngle{22}
% Preset sizes
\renewcommand{\LoopOnSmallState}{9.6} 		%float
\renewcommand{\LoopOnMediumState}{7}		%float : curvature
\renewcommand{\LoopOnLargeState}{5.8} 		%float
\renewcommand{\CLoopOnSmallState}{12}		%float
\renewcommand{\CLoopOnMediumState}{8}		%float
\renewcommand{\CLoopOnLargeState}{6}		%float
% Offset
\SetLoopOffset{0pt}
%
\MediumStates
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%\section{backward compatibility}%%%%%%
%%%%%  Obsolete commands from version 0.3, 0.4 and 1.0
%%%%%  kept for backward compatibility
%%%%%  cf users manual for description of compatibilty problems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\StateDimen}{outer}
\renewcommand{\StateDblDimen}{middle}
%
\renewcommand{\EdgeLabelPosit}{.45}   
\renewcommand{\EdgeLabelRevPosit}{.55}
\renewcommand{\ArcLabelPosit}{.40}
\renewcommand{\ArcLabelRevPosit}{.60}
\renewcommand{\LArcLabelPosit}{.40}
\renewcommand{\LArcLabelRevPosit}{.60}
\renewcommand{\LoopLabelPosit}{.25}
\renewcommand{\LoopLabelRevPosit}{.75}
\renewcommand{\CLoopLabelPosit}{.25}
\renewcommand{\CLoopLabelRevPosit}{.75}
%
\renewcommand{\LoopVarAngle}{28}
\renewcommand{\LoopOnVariableState}{5.1} 		%float
\renewcommand{\CLoopOnVariableState}{5.2}		%float
\setlength{\LoopVarOffset}{.7pt}
\renewcommand{\LoopOnVerySmallState}{15} 
% label position on initial-final arrow
\renewcommand{\InitStateLabelPosit}{.1}
\renewcommand{\InitStateLabelRevPosit}{.9}
\renewcommand{\FinalStateLabelPosit}{.9}
\renewcommand{\FinalStateLabelRevPosit}{.1}
%
\renewcommand{\ArrowOnVerySmallState}{5} 	%float
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \MediumStates
%%% Shape
%
%%% Variable States
\HorizontalStateVar\SelfAdjustState
%%% Showing -- hiding states
\ShowState
%%% Line
\renewcommand{\VSStateLineCoef}{.6} % coef. for very small state
%%% Background
%%% Label
%%% Label
\setlength{\VertexLineWidth}{0.6pt}             %% length
\renewcommand{\VertexLineColor}{black}        %% color
\renewcommand{\VertexBkgdStyle}{solid} 
\renewcommand{\VertexBkgdColor}{white}        %% color
\SetStateLabelColor{black}		
\renewcommand{\StateLabelScale}{1.7}
\renewcommand{\StateLabelSca}{1}% processing different from other parameters
\RigidLabel\FloatingLabel
%%% Initialisation
\RstState\RstVertex 
%%%%%%%%%%%%%%
%%%%%\section{edge parameters}%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetArcAngle{15}			%% int (degree)
\SetLArcAngle{30}			%% int (degree)
\SetArcCurvature{0.8}			%% float
\SetEdgeOffset{0pt}                     %% length
\SetArcOffset{1pt}			%% length
\SetLoopOffset{0pt}			%% length
\renewcommand{\ForthBackEdgeOffset}{5}	%% float : coef*\EdgeLineWidth -> offset
\FixEdgeBorder{2}{white}		%% int,color : coef*\EdgeLineWidth -> width of border
\FixEdgeLineDouble{0.5}{0.6}		%% float : coefs*\EdgeLineWidth -> (width of lines, distance)
%%%%%%%%%%%%%%
% ZZ aspect
%%%%%%%%%%%%%%
\setlength{\ZZSize}{.9cm}		% length : apparent diameter
\renewcommand{\ZZShape}{0.5}		% coef: opening of the ZZ
\SetZZLineWidth{1.7}			% float
\renewcommand{\TransLabelZZCoef}{0.6}	% float : coef*\ZZSize -> distance added for labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\InitStateLabelPosit}{.10}
\renewcommand{\InitStateLabelRevPosit}{.90}
\renewcommand{\FinalStateLabelPosit}{.90}
\renewcommand{\FinalStateLabelRevPosit}{.10}
% \SetEdgeArrowWidth{5pt}		%length of the edge arrow
% \SetEdgeArrowLengthCoef{1.4}		%float : coef*\EdgeArrowSizeDim width of EA
% \setlength{\EdgeDblArrowWidth}{5.5pt}		%length : size of EA for double transitions
% \renewcommand{\EdgeDblArrowLengthCoef}{1.7}	%int 
% \SetEdgeArrowInsetCoef{0.1}			%float : coef*\EdgeArrowSizeDim
% \SetEdgeArrowStyle{->}				%style (other styles : <-, |-|, -|,...)
% \renewcommand{\EdgeRevArrowStyle}{<-}           %style for reverse transitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initialization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetVCDirectory{}        %default dir=current dir
\HideFrame
\HideGrid
\MediumPicture
\HideName
\RigidLabel
\FullState				%% PlainState
\MediumStates

